Tangling and Braiding the Chessboard Complex

We describe a series of complexes that relate to the braid groups as the matching complexes relate to the symmetric groups. A modified construction applies as well to other complexes based on edge sets in graphs. We show that our constructions will yield Cohen-Macauley complexes provided the underlying complexes are Cohen-Macauley. Finally, we discuss a related series of complexes to provide some positive evidence that the braided Houghton groups, introduced by F. Degenhardt, are a series of groups with linearly increasing finiteness length as are the (unbraided) Houghton groups.

==> basic_notation.tex <==
%auto-ignore
\ProvidesFile{basic_notation.tex}[2001/09/20 KUB]

%
% This should be merged with buxmath.sty at some point
%

\newcommand{\congruent}{\equiv}


\newcommand{\DisplayOrList}[1]{%
  \ifNotationlisting
    \(#1\)%
  \else
    \[#1\]%
  \fi
}

%
% labelling defining occurences
%
\newcommand{\defnotion}[1]{%
  \begingroup
%    \def\tmp{#1}%
%    \expandafter\label\expandafter{\meaning\tmp}%
    \notion{#1}%
  \endgroup
}
\newcommand{\defref}[1]{%
  \begingroup
    \def\tmp{#1}%
    \expandafter\ref\expandafter{\meaning\tmp}%
  \endgroup
}
\newcommand{\defpref}[1]{%
  (\defref{#1})%
}
\newcommand{\locnotion}[1]{\emph{#1}}

%
% vertical =
%
\newcommand{\veq}{\shortparallel}

%
% set theory
%

\newcommand{\union}{\cup\OptIndex}
\newcommand{\symmetricdifference}{\mathbin{\triangle}}%{\mathbin{+_\Two}}
\newcommand{\intersect}[1][]{\cap_{#1}}
%\newcommand{\disjointunion}{\,\,\hbox to 0pt{$\hss\cdot\hss$}\hbox to 0pt{$\hss\union\hss$}\,\,}
\newcommand{\disjointunion}{\uplus}
\newcommand{\equalls}[1][]{%
  \IfEmptyThenElse{#1}{%
    =
  }{%
    =_{#1}
  }
}

\newcommand{\Parentheses}[1]{\left(#1\right)}
\newcommand{\Brakets}[1]{\left[#1\right]}
\newcommand{\ToThePower}[2]{#1^{#2}}
\newcommand{\AbsValue}[1]{\left|#1\right|}
\newcommand{\Factorial}[1]{#1!}

\newcommand{\EvalAt}{\negthinspace\Parentheses}
\newcommand{\ImageAt}{\negthinspace\Parentheses}
\newcommand{\ActOn}{\cdot}
\newcommand{\RestrictionTo}[1]{\left|_{#1}\right.}

\newcommand{\OpenInterval}[2]{\left(#1,#2\right)}
\newcommand{\ClosedInterval}[2]{\left[#1,#2\right]}
\newcommand{\RightOpenInterval}[2]{\left[#1,#2\right)}
\newcommand{\LeftOpenInterval}[2]{\left(#1,#2\right]}

\newcommand{\Binom}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}

\newcommand{\gobbleopt}[1][]{}

\newcommand{\forinf}{\exists^\infty}
\newcommand{\Forsome}[1]{\text{\ for some\ }#1}
\newcommand{\Forall}[1]{\text{\ for all\ }#1}
\newcommand{\Forinfmany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\ForSome}[1]{\qquad\text{\ for some\ }#1}
\newcommand{\ForAll}[1]{\qquad\text{\ for all\ }#1}
\newcommand{\ForInfMany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\For}[1]{\qquad\text{\ for\ }#1}
\newcommand{\Since}[1]{\qquad\text{\ since\ }#1}
\newcommand{\With}[1]{\qquad\text{\ with\ }#1}
\newcommand{\As}[1]{\qquad\text{\ as\ }#1}
\newcommand{\AND}{\qquad\text{\ and\ }\qquad}
%\newcommand{\OR}{\qquad\text{\ or\ }\qquad}
%\newcommand{\IF}{\qquad\text{\ if\ }\qquad}
\newcommand{\IFF}{\qquad\text{\ if and only if\ }\qquad}
\newcommand{\DefIff}{:\Longleftrightarrow}
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}
\newcommand{\Implies}{\ensuremath{\Longrightarrow}}

\newcommand{\ExtPowerOf}[2][]{%
  \ExtPot^{#1}\left(#2\right)
}
\newcommand{\tensor}[1][]{\otimes_{#1}}
\newcommand{\BilOf}[2][]{%
  \operatorname{Bil}_{#1}\negthinspace\left(#2\right)
}
\newcommand{\ExpOf}[2][]{\mathop{\exp_{#1}}\negthinspace\left(#2\right)}

\newcommand{\Diff}[1]{\mathrm{d}#1}
\newcommand{\Brace}[3]{%
  \left[#3\right]_{#1}^{#2}
}

\newcommand{\mapcolon}{:}

%
% Compound Notations
%
\makeatletter
\newcommand{\TwoByTwoMatrix}[4]{%
    \left(\begin{array}{cc}
      #1 & #2\\
      #3 & #4
    \end{array}\right)
}

\newcommand{\TwoByTwoDet}[4]{%
    \left|\begin{array}{cc}
      #1 & #2\\
      #3 & #4
    \end{array}\right|
}

\newcommand{\TwoColVector}[2]{%
    \left(\begin{array}{cc}
      #1\\
      #2
    \end{array}\right)
}

\newcommand{\TwoRwoVector}[2]{%
  \Parentheses{#1,#2}
}
\providecommand{\IfEmptyThenElse}[1]{%
  \begingroup
    \def\tempa{#1}%
    \def\tempb{}%
    \ifx\tempa\tempb
      \def\next{\@firstoftwo}%
    \else
      \def\next{\@secondoftwo}%
    \fi
  \expandafter\endgroup\next
}

\newcommand{\getfamfirstarg}[1][]{
  \def\tempa{#1}%
  \getfamsecondarg
}
\newcommand{\getfamsecondarg}[2][]{
  \def\tempb{#1}%
  \def\empty{}%
  \ifx\tempa\empty
    \left(#2\right)%
  \else
    \ifx\tempb\empty
      \left(#2\right)_{\tempa}%
    \else
      \left(#2\right)_{\tempa}^{\tempb}%
    \fi
  \fi
  \endgroup
}
\newcommand{\FamOf}{%
  \begingroup
    \getfamfirstarg
}
\iffalse
\newcommand{\FamOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left(#2\right)
  }{
    \left(#2\right)_{#1}
  }
}
\fi

\newcommand{\SetOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\{#2\right\}
  }{
    \left\{#1\,\,\vrule\,\,#2\right\}
  }
}

\newcommand{\GroupPresented}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\langle#2\right\rangle
  }{
    \left\langle#1\,\,\vrule\,\,#2\right\rangle
  }
}
\newcommand{\EquivClassOf}[2][]{\left[#2\right]_{#1}}
\newcommand{\TupelOf}[2][]{\left(#2\right)_{#1}}
\newcommand{\MaxOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \max\left(#2\right)
  }{
    \max_{#1}\left(#2\right)
  }
}

\newcommand{\MinOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \min\left(#2\right)
  }{
    \min_{#1}\left(#2\right)
  }
}

\newcommand{\InitTripleCommand}[2][]{%
  \begingroup
    \def\EndSymbol{#1}
    \def\TheSymbol{#2}%
    \getfirstarg
}
\newcommand{\getfirstarg}[1][]{%
    \def\tempa{#1}%
    \getlastargs
  }
\newcommand{\getlastargs}[2][]{%
    \def\tempb{#1}%
    \def\empty{}%
    \ifx\tempb\empty
      \ifx\tempa\empty
        \TheSymbol #2%
      \else
        \TheSymbol_{\tempa}#2%
      \fi
    \else
      \TheSymbol_{\tempa}^{#1}#2%
    \fi
  \endgroup
}

\newcommand{\Lim}[2][]{\lim_{#1}#2}

\newcommand{\Sum}[0]{\InitTripleCommand{\sum}}
\newcommand{\Int}[0]{\InitTripleCommand{\int}}
\newcommand{\Union}[0]{\InitTripleCommand{\bigcup}}
\newcommand{\Intersection}[0]{\InitTripleCommand{\bigcap}}
\newcommand{\DisUnion}[0]{\InitTripleCommand{{\biguplus}}}
\newcommand{\Product}[0]{\InitTripleCommand{\prod}}
\newcommand{\CoProduct}[0]{\InitTripleCommand{\coprod}}
\newcommand{\XProduct}[0]{\InitTripleCommand{\bigtimes}}
\newcommand{\FreeProd}[0]{\InitTripleCommand{\bigast}}
\newcommand{\BigJoin}[0]{\InitTripleCommand{\bigast}}
\newcommand{\DirectSum}[0]{\InitTripleCommand{\bigoplus}}
\newcommand{\Min}[0]{\InitTripleCommand{\min}}
\newcommand{\Max}[0]{\InitTripleCommand{\max}}
\newcommand{\Inf}[0]{\InitTripleCommand{\inf}}
\newcommand{\InfOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \inf#2
  }{
    \inf_{#1}#2
  }
}
\newcommand{\Sup}[0]{\InitTripleCommand{\sup}}
\newcommand{\SupOf}{\sup}

\newcommand{\MatrixOf}[2][]{%
  \IfEmptyThenElse{#1}{%
    \left(#2\right)
  }{%
    \left(#2\right)_{#1}
  }
}

\newcommand{\OrderOf}{\operatorname{ord}\OptIndexParentheses}

\newcommand{\TensorProduct}[3][]{%
  \IfEmptyThenElse{#1}{
    #2\otimes#3
  }{
    #2\otimes_{#1}#3
  }
}

\newcommand{\leftsemidirectprod}[1][]{%
  \rtimes\OptIndex[#1]
}

\newcommand{\wreathprod}{\wr}

\newcommand{\ColumnVector}[1]{%
  \left(\begin{array}{c}
    #1
  \end{array}\right)
}

\newcommand{\Interval}[2]{\left[#1,#2\right]}

% \makeatletter
% \def\@lap[#1,#2]#3{%
%   \parbox[b][0pt][b]{0pt}{%
%     \raisebox{#2}{%
%       \parbox[b][0pt][c]{0pt}{%
%          \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
%       }%
%     }%
%   }%
%   \ignorespaces
% }%
% \newcommand{\clap}[2][0pt,0pt]{\@lap[#1]{#2}}
% \makeatother

\newcommand{\clap}[1]{\makebox[0pt][c]{#1}}


\newcommand{\PreImage}[2]{{#1}^{-1}\left(#2\right)}
%
%
%
\newcommand{\IfNonEmpty}[2]{\IfEmptyThenElse{#1}{}{#2}}
\newcommand{\OptExponent}[1][]{\IfNonEmpty{#1}{^{#1}}}
\newcommand{\OptParExponent}[1][]{\IfNonEmpty{#1}{^{\left(#1\right)}}}
\newcommand{\OptIndex}[1][]{\IfNonEmpty{#1}{_{#1}}}
\newcommand{\OptArg}[2]{#1\IfNonEmpty{#2}{\EvalAt{#2}}}
\newcommand{\OptIndexOptPar}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParentheses}
\newcommand{\OptParentheses}[1][]{\IfNonEmpty{#1}{\negthinspace\left(#1\right)}}
\newcommand{\OptExponentParentheses}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAt}
\newcommand{\OptIndexParentheses}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentParentheses}
\newcommand{\OptIndexParExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParExponent}
\newcommand{\OptIndexExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponent}
\newcommand{\DoubleArg}[2]{\EvalAt{#1,#2}}
\newcommand{\OptExponentDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\DoubleArg}
\newcommand{\OptIndexDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentDoubleArg}
\newcommand{\newconst}[2]{%
  \newcommand{#1}[0]{#2}
  }
\newcommand{\newvariable}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\renewvariable}[2]{%
  \renewcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\renewcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\tmpvariable}[2]{%
  \let#1\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Of\endcsname\undefined
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\newparexpvariable}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
  }
\newcommand{\newmap}[2]{%
  \newcommand{#1}[1][]{\OptArg{#2}{##1}}
  }
\newcommand{\newindexedmap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptParentheses}
  }
\newcommand{\NewMap}[2]{%
  \newvariable{#1}{#2}%
  \begingroup
    \escapechar=-1%
    \expandafter\global\expandafter\newcommand\expandafter{\csname \string#1Of\endcsname}{#2\OptIndexParentheses}
  \endgroup
}
\newcommand{\newMap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\EvalAt}
  }
\newcommand{\newMapTwo}[2]{%
  \newcommand{#1}[2]{#2\left(##1,##2\right)}
  }
\newcommand{\newMapTWO}[2]{%
  \newcommand{#1}[2]{#2\left(##1;##2\right)}
  }
\newcommand{\newexpvector}[2]{%
  \newcommand{#1}{#2\OptParExponent}
  }

\newcommand{\newexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexExponent}
}
\newcommand{\newparexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
}
\newcommand{\OR}{\quad\text{or}\quad}
%
% picture
%
  \newcommand{\drawpath}[1]{%
    \begingroup%
      \edef\tempa{#1}%
      \expandafter\drawline\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\dashpath}[2]{%
    \begingroup%
      \edef\tempa{#2}%
      \def\tempb{\dashline[0]{#1}}%
      \expandafter\tempb\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\plot}[2]{%
    \expandafter\put#1{#2}\ignorespaces
  }
  \def\lap[#1,#2]#3{%
    \parbox[b][0pt][b]{0pt}{%
      \raisebox{#2}{%
        \parbox[b][0pt][c]{0pt}{%
           \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
        }%
      }%
    }%
    \ignorespaces
  }%
  \newcommand{\Bullet}[2][0mm,0mm]{%
    \lap[0mm,0mm]{$\bullet$}
    \lap[#1]{$#2$}
  }

\newcommand{\UnitsOf}[1]{#1^{*}}
\newcommand{\ThePullback}[1]{#1^{*}\OptParentheses}

\newcommand{\DirectedSystem}[3][]{%
  \IfEmptyThenElse{#1}{%
    (#2)_{#3}
  }{%
    (#2)_{#1\in#3}%
  }%
}

\newcommand{\Morph}[3][]{%
  \IfEmptyThenElse{#1}{%
    \mathop{\mathrm{Mor}}\left(#2,#3\right)%
  }{%
    \mathop{\mathrm{Mor}}\limits_{#1}\left(#2,#3\right)%
  }%
}
\newcommand{\InvLimit}[2][]{\mathop{\inverslim}_{#1}#2}
\newindexedmap{\InvLimitMap}{\pi}
\newmap{\InvUnivMap}{\iota}
\newcommand{\DirLimit}[2][]{\mathop{\directlim}_{#1}#2}
\newindexedmap{\DirLimitMap}{\iota}
\newmap{\DirUnivMap}{\pi}
\newcommand{\Limit}[2][]{\mathop{\lim}_{#1}#2}

\newcommand{\HoColimOf}[1]{%
  \operatorname{ho-colim}\left(#1\right)
}

\newcommand{\FunctorMap}[1]{#1_{*}\OptParentheses}
\newvariable{\TheGraphLift}{\tilde{\TheGraph}}
\newcommand{\graphminus}{-}
\newvariable{\TheEdgeLift}{\tilde{\TheEdge}}

%
% small integers
%
\newcommand{\Number}[1]{#1}
\newvariable{\Zero}{\Number{0}}
\newvariable{\One}{\Number{1}}
\newvariable{\qOne}{1}
\newvariable{\OneHalf}{\ensuremath{\frac{1}{2}}}
\newvariable{\Two}{\Number{2}}
\newvariable{\Three}{\Number{3}}
\newvariable{\Four}{\Number{4}}
\newvariable{\Five}{\Number{5}}
\newvariable{\Six}{\Number{6}}
\newvariable{\Seven}{\Number{7}}
\newvariable{\Eight}{\Number{8}}
\newvariable{\Nine}{\Number{9}}
\newvariable{\Ten}{\Number{10}}


\endinput


==> bibliography.tex <==
%auto-ignore
\ProvidesFile{bibliography.tex}[2001/10/16 KUB]
\begin{references}%
  \newcommand{\BielPre}[2]{%
    Preprint series #1 -- #2, SFB~343; Bielefeld (19#1)%
  }%
  \begin{article}{Abel79}{Abels:1979}%
    \au{H.~Abels}
    \ti{An example of a finitely presented solvable group}
    \lo{In \cite{Wall:1979}}{205 -- 211}
  \end{article}
  \begin{book}{Abel87}{Abels:1987}%
    \au{H.~Abels}
    \ti{Finite presentability of $S$-arithmetic groups -- Compact
        presentability of solvable groups}
    \lo{Springer LNM~1261 (1987)}{}
  \end{book}
  \begin{article}{Abel91}{Abels:1991}
    \au{H.~Abels}
    \ti{Finiteness Properties of certain arithmetic groups in the function field case}
    \lo{Israel J.\ Math.\ 76 (1991)}{113 -- 128}
  \end{article}
  \begin{article}{AbBr87}{Abels.Brown:1987}
    \au{H.~Abels, K.S.~Brown}
    \ti{Finiteness Properties of Solvable $S$-Arithmetic Groups: An Example}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{77 -- 83}
  \end{article}
  \begin{article}{AbHo93}{Abels.Holz:1993}
    \au{H.~Abels, S.~Holz}
    \ti{Higher Generation by Subgroups}
    \lo{Journal of Algebra 160 (1993)}{310 -- 341}
  \end{article}
  \begin{article}{AbTi97}{Abels.Tiemeyer:1997}%
    \au{H.~Abels, A.~Tiemeyer}
    \ti{Compactness Properties of Locally Compact Groups}
    \lo{Transformation Groups 2 (1997)}{119 - 135}
%    (confer~\cite{Tiemeyer:1997})
  \end{article}
  \begin{article}{\AA{}ber86}{Aberg:1986}%
    \au{H.~\AA{}berg}
    \ti{Bieri-Strebel Valuations (of Finite Rank)}
    \lo{Proceedings of the London Mathematical Society 52 (1986)}{269 -- 304}
  \end{article}
  \begin{article}{Abra95}{Abramenko:review:1995}
    \au{P.~Abramenko}
    \ti{Review 95e:20049 on \cite{Abels.Holz:1993}}
    \lo{Mathematical Reviews (1995)}{}
  \end{article}
  \begin{thesis}{Abra87}{Abramenko:1987}
    \au{P.~Abramenko}
    \ti{Endlichkeitseigenschaften der Gruppen $\SL_n(\FFF_q[t])$}
    \lo{Thesis Frankfurt am Main (1987)}{}
  \end{thesis}
  \begin{notes}{Abra94}{Abramenko:1994}
    \au{P.~Abramenko}
    \ti{{\selectlanguage{german}Chevalleygruppen}}
    \lo{Manuscript (Frankfurt, WS~1994/95)}{}
  \end{notes}
  \begin{thesis}{Abra95}{Abramenko:1995}%
    \au{P.~Abramenko}
    \ti{Twin Buildings, Spherical buildings and Finiteness
        Properties of Almost Simple $\FFF_q$-Groups over
        $\FFF_q[t]$}
    \lo{Habilitation thesis (Frankfurt, 1995)}{}
  \end{thesis}
  \begin{book}{Abra96}{Abramenko:1996}%
    \au{P.~Abramenko}
    \ti{Twin Buildings and Applications to $S$-Arithmetic Groups}
    \lo{Springer LNM~1641 (1996)}{}
  \end{book}
  \begin{preprint}{Abra99}{Abramenko:unpublished}
    \au{P.~Abramenko}
    \ti{??}
    \lo{??}{}
  \end{preprint}
  \begin{article}{Akit01}{Akita:2001}
    \au{T.~Akita}
    \ti{Homological infiniteness of Torelli groups}
    \lo{Topology 40 (2001), no. 2}{213 -- 221}
  \end{article}
  \begin{article}{Alon94}{Alonso:1994}
    \au{J.~Alonso}
    \ti{Finiteness conditions on groups and quasi-isometries}
    \lo{Journal of Pure and Applied Algebra 95 (1994)}{121 -- 129}
  \end{article}
  \begin{book}{Alpe91}{Alperin:1991}
    \ed{R.~Alperin}
    \ti{Arboreal Group Theory}
    \lo{MSRI Publications 19 (Springer, 1991)}{}
  \end{book}
  \begin{article}{BBLSW99}{Babson.Bjoerner.Linusson.Shareshian.Welker:1999}%
    \au{E.~Babson, A.~Bj\"{o}rner, S.~Linusson, J.~Shareshian, V.~Welker}
    \ti{Complexes of Not $i$-Connected Graphs}
    \lo{Topology 38(2) (1999)}{271 -- 299}
  \end{article}
  \begin{article}{BGS01}{Bartholdi.Grigorchuk.Sunik:2001}%
    \au{L.~Bartholdi, R.I.~Grigorchuk, Z.~\v{S}uni\'{k}}
    \ti{Branch Groups}
    \lo{preprint (2001)}{}
  \end{article}
  \begin{article}{BBN59}{Baumslag.Boone.Neumann:1959}%
    \au{G.~Baumslag, W.W.~Boone, B.H.~Neumann}
    \ti{Some Unsolvable Problems About Elements and Subgroups of Groups}
    \lo{Mathematica Scandinavica 7 (1959)}{191 -- 201}
  \end{article}
  \begin{article}{Behr62}{Behr:1962}%
    \au{H.~Behr}
    \ti{{\selectlanguage{german}\"U{}ber die endliche Definierbarkeit von Gruppen}}
    \lo{{\selectlanguage{german}Journal f\"u{}r die reine und angewandte
        Mathematik (Crelles Journal) 211 (1962)}}{116 -- 122}
  \end{article}
  \begin{article}{Behr68}{Behr:1968}%
    \au{H.~Behr}
    \ti{{\selectlanguage{german}Zur starken Approximation in algebraischen Gruppen \"u{}ber globalen
        K\"o{}rpern}}
    \lo{{{\selectlanguage{french}Journal f\"u{}r die reine und angewandte
        Mathematik (Crelles Journal) 229 (1968)}}}{107 -- 116}
  \end{article}
  \begin{preprint}{Behr98}{Behr:1998}%
    \au{H.~Behr}
    \ti{Arithmetic groups over function fields I\null.
        A complete
        characterization of finitely generated and finitely presented
        arithmetic subgroups of reductive algebraic groups}
    \lo{{\selectlanguage{german}Journal f\"u{}r die reine und
        angewandte Mathematik (Crelles Journal) 495 (1998)}}{79--118}
  \end{preprint}
  \begin{preprint}{Behr99}{Behr:1999}
    \au{H.~Behr}
    \ti{Higher finiteness properties of $S$-arithmetic groups in the function field case I: Chevalley groups with coefficients in $\FFF_q[t]$}
    \lo{Preprint, Frankfurt (1999)}{}
  \end{preprint}
  \begin{preprint}{BeBr03}{Belk.Brown:2003}
    \au{J.M.~Belk, K.S.~Brown}
    \ti{Forest Diagrams for Elements of Thompson's Group $F$}
    \lo{Preprint (2003), arXiv:math.GR/0305412}{}
  \end{preprint}
  \begin{preprint}{BeBu02a}{Belk.Bux:2002a}
    \au{J.M.~Belk, K.-U.~Bux}
    \ti{Flows, Robots, and Amenability} % A Max-Flow-Min-Cut Theorem for Infinite Graphs and Applications to Amenability}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{preprint}{BeBu02b}{Belk.Bux:2002b}
    \au{J.M.~Belk, K.-U.~Bux}
    \ti{Thompson's Group $F$ is not Minimally Almost Convex}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{preprint}{BeBu03}{Belk.Bux:2003}
    \au{J.M.~Belk, K.-U.~Bux}
    \ti{Thompson's Group $F$ is not Minimally Almost Convex}
    \lo{Preprint, arXiv:math.GR/0301141}{}
  \end{preprint}
  \begin{preprint}{BeBu02c}{Belk.Bux:2002c}
    \au{J.M.~Belk, K.-U.~Bux}
    \ti{A Series of Groups Related to Thompson's Groups $F$ and $T$}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{article}{BeBr97}{Bestvina.Brady:1997}%
    \au{M.~Bestvina, N.~Brady}
    \ti{Morse theory and finiteness properties of groups}
    \lo{Inventiones mathematicae 129 (1997)}{445 -- 470}
  \end{article}
  \begin{article}{BeFe00}{Bestvina.Feighn:2000}
    \au{M.~Bestvina, M.~Feighn}
    \ti{The topology at infinity of $\Out(F_n)$}
    \lo{Inventiones mathematicae 140 (2000)}{651 -- 692}
  \end{article}
  \begin{article}{BFH00a}{Bestvina.Feighn.Handel:2000a}
    \au{M.~Bestvina, M.~Feighn, M.~Handel}
    \ti{The Tits Alternative for $\operatorname{Out}(F_n)$ I: Dynamics of exponentially growing automorphisms}
    \lo{Annals of Mathematics 151 (2000)}{517 -- 623}
  \end{article}
  \begin{preprint}{BFH00b}{Bestvina.Feighn.Handel:2000b}
    \au{M.~Bestvina, M.~Feighn, M.~Handel}
    \ti{The Tits Alternative for $\operatorname{Out}(F_n)$ II: A Kolchin Theorem}
    \lo{preprint}{}
  \end{preprint}
  \begin{article}{Bier99}{Bieri:1999}%
    \au{R.~Bieri}
    \ti{Finiteness length and connectivity length for groups}
    \lo{In \cite{Cossey.Miller.Neumann.Shapiro:1999}}
         {9 -- 22}
  \end{article}
  \begin{article}{BiEc74}{Bieri.Eckmann:1974}
    \au{R.~Bieri, B.~Eckmann}
    \ti{Finiteness Properties of Duality Groups}
    \lo{Commentarii Mathematici Helvetici 49 (1974)}{74 -- 83}
  \end{article}
  \begin{preprint}{BiGe98}{Bieri.Geoghegan:1998}%
    \au{R.~Bieri, R.~Geoghegan}
    \ti{Connectivity properties of group actions on non-positively
        curved spaces~II: The geometric invariants}
    \lo{Preprint (Frankfurt, October~1998)}{}
  \end{preprint}
  \begin{preprint}{BiHa00}{Bieri.Harlander:2000}
    \au{R.~Bieri, J.~Harlander}
    \ti{On the FP$_3$-Conjecture for Metabelian Groups}
    \lo{Preprint (Frankfurt, 2000)}{}
  \end{preprint}
  \begin{article}{BiRe88}{Bieri.Renz:1988}%
    \au{R.~Bieri, B.~Renz}
    \ti{Valuations on free resolutions and higher geometric
        invariants of groups}
    \lo{Commentarii Mathematici Helvetici 63 (1988)}{464 -- 497}
  \end{article}
  \begin{article}{BiSt80}{Bieri.Strebel:1980}
    \au{R.~Bieri, R.~Strebel}
    \ti{Valuations and Finitely Presented Metabelian Groups}
    \lo{Proceedings of the London Mathematical Society 41 (1980)}{439 -- 464}
  \end{article}
  \begin{manuscript}{BiSt}{Bieri.Strebel:nodate}
    \au{R.~Bieri, R.~Strebel}
    \ti{On Groups of PL-Homemorphisms of the Real Line}
    \lo{Unpublished Manuscript}{}
  \end{manuscript}
  \begin{preprint}{BiSt92}{Bieri.Strebel:1992}
    \au{R.~Bieri, R.~Strebel}
    \ti{Geometric Invariants of Discrete Groups}
    \lo{Preprint (Frankfurt, 1992)}{}
  \end{preprint}
  \begin{article}{Bj\"{o}r92}{Bjoerner:1992}
    \au{A.~Bj\"orner}
    \ti{The Homology and Shellability of Matroids and Geometric Lattices}
%    \lo{in \ed{N.~White (ed.)} \ti{Matroid Applications}
%        (Cambridge University Press 1992)}{ 226 -- 283}
    \lo{In \cite{White:1992}}{226 -- 283}
  \end{article}
  \begin{article}{BLVZ94}{Bjoerner.Lovasz.Vrecica.Zivaljevic:1994}%
    \au{A.~Bj\"orner, L.~Lov\'{a}sz, S.T.~Vre\'{c}ica, R.T.~\v{Z}ivaljevi\'{c}}
    \ti{Chessboard complexes and matching complexes}
    \lo{Journal of the London Mathematical Society 49 (1994)}{25 -- 39}
  \end{article}
  \begin{article}{Bore62}{Borel:1962}%
    \au{A.~Borel}
    \ti{Arithmetic properties of linear algebraic groups}
    \lo{Proceeding of the International Congress of Mathematicians, Stockholm, 1962
        (Upsala 1963)}{10 -- 22}
  \end{article}
  \begin{article}{Bore63}{Borel:1963}%
    \au{A.~Borel}
    \ti{Some finiteness properties of adele groups over number fields}
    \lo{Publ.\ Math., Inst.\ Hautes Etud.\ Sci.\ 16 (1963)}{5 -- 30}
  \end{article}
  \begin{book}{Bore91}{Borel:1991}%
    \au{A.~Borel}
    \ti{Linear Algebraic Groups}
    \edition{Second Enlarged Edition}
    \lo{Springer GTM 126, New York (1991)}{}
  \end{book}
  \begin{article}{BoHa62}{Borel.Harish-Chandra:1962}%
    \au{A.~Borel, Harish-Chandra}
    \ti{Arithmetic subgroups of algebraic groups}
    \lo{Annals of Mathematics 75 (1962)}{485 -- 535}
  \end{article}
  \begin{article}{BoSe73}{Borel.Serre:1973}%
    \au{A.~Borel, J-P.~Serre}
    \ti{Corners and arithmetic groups}
    \lo{Commentarii Mathematici Helvetici 48 (1973)}{436 -- 491}
  \end{article}
  \begin{article}{BoSe76}{Borel.Serre:1976}%
    \au{A.~Borel, J.-P.~Serre}
    \ti{{\selectlanguage{french}Cohomologie d'immeubles et de groupes S-arithm\'{e}tiques}}
    \lo{Topology 15 (1976)}{211 -- 232}
  \end{article}
  \begin{article}{BoTi65}{Borel.Tits:1965}%
    \au{A.~Borel, J.~Tits}
    \ti{Groupes r\'{e}ductifs}
    \lo{Publ.\ Math., Inst.\ Hautes Etud.\ Sci.\ 27 (1965)}{55 -- 150}
  \end{article}
  \begin{article}{Brid00}{Bridson:2000}
    \au{M.~Bridson}
    \ti{Finiteness Properties for Subgroups of $\GL(n,\ZZZ)$}
    \lo{Math. Annalen., 317 (2000)}{629 -- 633}
  \end{article}
  \begin{book}{BrHa99}{Bridson.Haefliger:1999}
    \au{M.R.~Bridson, A.~Haefliger}
    \ti{Metric Spaces of Non-Positive Curvature}
    \lo{{\selectlanguage{german}Grundlehren der Mathematischen Wissenschaften} (Springer, 1999)}{}
  \end{book}
  \begin{article}{BrVo01}{Bridson.Vogtmann:2001}
    \au{M.~Bridson, K.~Vogtmann}
    \ti{The symmetries of Outer space}
    \lo{Duke Mathematical Journal 106 (2001), no. 2}{391 -- 409}
  \end{article}
  \begin{book}{Brow82}{Brown:1982}%
    \au{K.S.~Brown}
    \ti{Cohomology of Groups}
    \lo{Springer GTM 87, New York (1982)}{}
  \end{book}
  \begin{article}{Bro87a}{Brown:1987a}%
    \au{K.S.~Brown}
    \ti{Finiteness Properties of Groups}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{45 -- 75}
  \end{article}
  \begin{article}{Bro87b}{Brown:1987b}%
    \au{K.S.~Brown}
    \ti{Trees, valuations, and the Bieri-Neumann-Strebel invariant}
    \lo{Inventiones mathematicae 90 (1987)}{479 -- 504}
  \end{article}
  \begin{book}{Brow89}{Brown:1989}
    \au{K.S.~Brown}
    \ti{Buildings}
    \lo{Springer, New York, Berlin (1989)}{}
  \end{book}
  \begin{article}{BrGe84}{Brown.Geoghegan:1984}%
    \au{K.S.~Brown, R.~Geoghegan}
    \ti{An infinite-dimensional torsion-free $FP_\infty$ group}
    \lo{Inventiones mathematicae 77 (1984)}{367 -- 381}
  \end{article}
  \begin{report}{BrTi72}{Bruhat.Tits:1972}%
    \au{F.~Bruhat, J.~Tits}
    \ti{{\selectlanguage{french}Groupes R\'{e}ductives sur un Corps Local I}}
    \lo{{\selectlanguage{french}Publications Math\'{e}matiques IHES 41 (1972)}}{5 -- 252}
  \end{report}
  \begin{article}{BBW79}{Brunner.Burns.Wiegold:1979}
    \au{A.M.~Brunner, R.G.~Burns, J.~Wiegold}
    \ti{On the Number of Quotients, of One Kind or Another, of the Modular Group}
    \lo{Mathematical Scientist 4 (1979)}{93 -- 98}
  \end{article}
  \begin{article}{BuGo99}{Bux.Gonzalez:1999}
    \au{K-U.~Bux, C.R.~Gonzalez}
    \ti{The Bestvina-Brady Construction Revisited -- Geometric Computation
        of $\Sigma$-Invariants for Right Angled Artin Groups}
    \lo{Journal of the London Mathematical Society (2) 60 (1999)}{793 -- 801}
%    \url{http://www.math.utah.edu/\~{}bux/math/bugo97.ps.gz}
  \end{article}
  \begin{article}{Bux97a}{Bux:1997a}%
    \au{K.-U.~Bux}
    \ti{Finiteness Properties of some Metabelian $S$-Arithmetic Groups}
    \lo{Proceedings of the London Mathematical Society 75 (1997)}{308 -- 322}
  \end{article}
  \begin{thesis}{Bux97b}{Bux:1997b}%
    \au{K.-U.~Bux}
    \ti{{\selectlanguage{german}Endlichkeitseigenschaften auf"|l\"o{}sbarer
        arithmetischer Gruppen \"u{}ber Funktionenk\"o{}rpern}}
    \lo{PhD thesis (Frankfurt, 1997)}{}
%    \url{http://www.math.uni-frankfurt.de/\~{}bux/math/bux98.ps.gz}
  \end{thesis}
  \begin{article}{Bux02}{Bux:2002}
    \au{K-U.~Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups over Global
        Function Fields}
    \lo{Preprint (2002)}{}
%    \url{http://www.math.utah.edu/\~{}bux/math/bux99b.ps.gz}
  \end{article}
  \begin{article}{Bux99b}{Bux:1999b}
    \au{K.-U.~Bux}
    \ti{Orbit spaces of subgroup complexes, Morse Theory, and a new proof of a conjecture of Webb}
    \lo{Topology Proceedings 24 (Spring 1999)}{39 -- 51}
  \end{article}
  \begin{article}{Bux99}{Bux:1999}
    \au{K.-U.~Bux}
    \ti{Orbit spaces of subgroup complexes, Morse Theory, and a new proof of a conjecture of Webb}
    \lo{Topology Proceedings 24 (Spring 1999)}{39 -- 51}
  \end{article}
  \begin{preprint}{Bux01}{Bux:2001}
    \au{K.-U.~Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups -- a Survey}
    \lo{To appear in Proceedings ``Groups: Geometric and Combinatorial Aspects'' (Bielefeld, 1999)}{}
    \url{http://www.math.cornell.edu/\~{}bux/math/bux99d.ps.gz}
  \end{preprint}
  \begin{article}{Bux03a}{Bux:2003a}
    \au{K-U.~Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups over Global
        Function Fields}
    \lo{%
      Submitted to Geometry and Topology (2003)
      arXiv:math.GR/0212365}{}
%    \url{http://www.math.utah.edu/\~{}bux/math/bux99b.ps.gz}
  \end{article}
  \begin{preprint}{Bux03b}{Bux:2003b}
    \au{K.-U.~Bux}
    \ti{Brading and Tangling the Chessboard Complex}
    \lo{Preprint, arXiv:???}{}
  \end{preprint}
  \begin{article}{Cann87}{Cannon:1987}
    \au{J.W.~Cannon}
    \ti{Almost convex groups}
    \lo{Geometriae Dedicata 22 (1987)}{197 -- 210}
  \end{article}
  \begin{article}{CFGT89}{Cannon.Floyd.Grayson.Thurston:1989}
    \au{J.W.~Cannon, W.J.~Floyd, M.A.~Grayson, W.P.~Thurston}
    \ti{Solvgroups are not Almost Convex}
    \lo{Geometria Dedicata 31 (1989)}{291 -- 300}
  \end{article}
  \begin{article}{CFP96}{Cannon.Floyd.Parry:1996}
    \au{J.W.~Cannon, W.J.~Floyd, W.R.~Parry}
    \ti{Introductory Notes to Richard~Thompson's Groups}
    \lo{L'Enseignement Math\'{e}matique 42 (1996)}{215 -- 256}
  \end{article}
  \begin{book}{CaFr67}{Cassels.Froehlich:1967}
    \ed{J.W.S.~Cassels, A.~Fr\"o{}hlich}
    \ti{Algebraic Number Theory. Proceedings of an Instructional
        Conference organized by the London Mathematical Society
        (A Nato Advanced Study Institute)
        with Support of the International Mathematical Union}
    \lo{Academic Press, London (1967)}{}
   \end{book}
  \begin{article}{Chev60}{Chevalley:1960}%
    \au{C.~Chevalley}
    \ti{{\selectlanguage{french}Certain Sch\'{e}mas de Groupes Semi-Simples}}
    \lo{{\selectlanguage{french}S\'{e}minaire Bourbaki 13e ann\'{e}e (1960/61) n$\circ$~219}}{1 -- 16}
  \end{article}
  \begin{article}{Chou80}{Chou:1980}
    \au{C.~Chou}
    \ti{Elementary amenable groups}
    \lo{Illinois Journal of Mathematics 24 (1980)}{396 -- 407}
  \end{article}
  \begin{preprint}{ClTa02}{Cleary.Taback:2002}
    \au{S.~Cleary, J.~Taback}
    \ti{Thompson's Group $F$ is not Almost Convex}
    \lo{Preprint (2002), to appear: Journal of Algebra}{}
  \end{preprint}
  \begin{book}{CMNS99}{Cossey.Miller.Neumann.Shapiro:1999}
      \ed{J.~Cossey, C.F.~Miller, W.~Neumann and M.~Shapiro}
      \ti{Geometric Group Theory down under}
      \lo{Proc.\ of the special year on geometric group theory,
          Australia Nat.\ Univ.\ Canberra, 1996 (de Gruyter, 1999)}{}
  \end{book}
  \begin{article}{CuMo87}{Culler.Morgan:1987}
    \au{M.~Culler, K.~Vogtmann}
    \ti{Group Actions on $\RRR$-Trees}
    \lo{Proceedings of the London Mathematical Society 35 (1987)}{571 -- 604}
  \end{article}
  \begin{article}{CuVo86}{Culler.Vogtmann:1986}
    \au{M.~Culler, K.~Vogtmann}
    \ti{Moduli of graphs and automorphisms of free groups}
    \lo{Inventiones mathematicae 84 (1986)}{91 -- 119}
  \end{article}
  \begin{article}{DaSh91}{Davis.Shapiro:1991}
    \au{M.W.~Davis, M.~Shapiro}
    \ti{Coxeter Groups are Almost Convex}
    \lo{Geometria Dedicata 39 (1991)}{55 -- 57}
  \end{article}
  \begin{thesis}{Dege00}{Degenhardt:2000}
    \au{F.~Degenhardt}
    \ti{{\selectlanguage{german}Endlichkeitseigenschaften gewisser
         Gruppen von Z\"{o}pfen unendlicher Ordnung}}
    \lo{PhD thesis (Frankfurt, 2000)}{}
  \end{thesis}
  \begin{book}{DiDu89}{Dicks.Dunwoody:1989}
    \au{W.~Dicks, M.J.~Dunwoods}
    \ti{Groups acting on graphs}
    \lo{Cambridge studies in advanced mathematics 17 (Cambridge University Press, 1989)}{}
  \end{book}
  \begin{article}{EiGa57}{Eilenberg.Ganea:1957}
    \au{S.~Eilenberg, T.~Ganea}
    \ti{On the Lusternik-Schnirelmann category of abstract groups}
    \lo{Annals of Mathematics 65 (1957)}{517 -- 518}
  \end{article}
  \begin{book}{Eggl58}{Eggleston:1958}%
    \au{H.G.~Eggleston}
    \ti{Convexity}
    \lo{Cambridge Tracts in Mathematics and Mathematical Physics, Cambridge (1958)}{}
  \end{book}
  \begin{preprint}{ElHe02}{Elder.Hermiller:2002}
    \au{M.~Elder, S.~Hermiller}
    \ti{Minimal almost convexity: some examples.}
    \lo{in preparation}{}
  \end{preprint}
  \begin{article}{Epst62}{Epstein:1962}
    \au{D.B.A.~Epstein}
    \ti{Ends}
    \lo{in \cite{Fort:1962}}{110 -- 117}
  \end{article}
  \begin{article}{FaNe62}{Fadell.Neuwirth:1962}
    \au{E.~Fadell, L.~Neuwirth}
    \ti{Configuration Spaces}
    \lo{Mathematica Scandinavica 10 (1962)}{111 -- 118}
  \end{article}
  \begin{thesis}{Ford95}{Fordham:1995}
    \au{S.B.~Fordham}
    \ti{Minimal Length Elements of Thompson's Group $F$}
    \lo{PhD Thesis (Brigham Young University, 1995)}{}
  \end{thesis}
  \begin{article}{For98a}{Forman:1998a}
    \au{R.~Forman}
    \ti{Morse theory for cell complexes}
    \lo{Advances in Mathematics 134 (1998)}{90 -- 145}
  \end{article}
  \begin{article}{For98b}{Forman:1998b}
    \au{R.~Forman}
    \ti{Witten-Morse theory for cell complexes}
    \lo{Topology 37 (1998)}{945 --979}
  \end{article}
  \begin{book}{Fort62}{Fort:1962}%
    \ed{M.K.~Fort}
    \ti{Topology of 3-Manifolds}
    \lo{Proceedings of The University of Georgia Institute (1961), Prentice-Hall 1962}{}
  \end{book}
  \begin{book}{GHV90}{Ghys.Haefliger.Verjovsky:1990}%
    \ed{E.~Ghys, A.~Haefliger, A.~Verjovsky}
    \ti{Groups from a geometric viewpoint}
    \lo{Proceedings of the workshop held in Trieste, March 26--April 6, 1990}{World Sci. Publishing, 1991}
  \end{book}
  \begin{article}{Grig80}{Grigorchuk:1980}
    \au{R.I.~Grigorchuk}
    \ti{On Burnside's Problem on periodic groups}
    \lo{Functional Analysis Applications 14 (1980)}{41 -- 43}
  \end{article}
  \begin{article}{Grig85}{Grigorchuk:1985}
    \au{R.I.~Grigorchuk}
    \ti{On the growth degrees of $p$-groups and torsion free groups}
    \lo{Math. USSR Sbornik 54 (1986)}{185 -- 205}
  \end{article}
  \begin{article}{Gri98}{Grigorchuk:1998}
    \au{R.I.~Grigorchuk}
    \ti{An example of a finitely presented amenable group not belonging to the class $EG$}
    \lo{Math. USSR Sbornik 189 (1998)}{75 -- 95}
  \end{article}
  \begin{article}{GrWi00}{Grigorchuk.Wilson:2000}
    \au{R.I.~Grigorchuk, J.S.~Wilson}
    \ti{The Conjugacy Problem for Certain Branch Groups}
    \lo{Proceedings of the Steklov Institute of Mathematics 231 (2000)}{204 -- 219}
  \end{article}
  \begin{article}{Grom81}{Gromov:1981}
    \au{M.~Gromov}
    \ti{Groups of Polynomial Growth and Expanding Maps}
    \lo{Publicationes Mathematicae IHES 53 (1981)}{53 -- 73}
  \end{article}
  \begin{book}{GrRo84}{Gruenberg.Roseblade:1984}
    \ed{K.W.~Gruenberg, J.E.~Roseblade}
    \ti{Group Theory: Essays for Philip Hall}
    \lo{Academic Press (1984)}{}
  \end{book}
  \begin{article}{Grus40}{Grushko:1940}
    \au{I.A.~Grushko}
    \ti{{\selectlanguage{german}^^dcber die Basen eines freien Produktes von Gruppen} (Russian, with German summary)}
    \lo{Mat. Sb. 8 (1940)}{169 -- 182}
  \end{article}
  \begin{preprint}{Guba02a}{Guba:2002a}
    \au{V.S.~Guba}
    \ti{The Dehn Function of Richard Thompson's Group $F$ is Quadratic}
    \lo{Preprint (2002), arXiv:math.GR/0211395 v1}{}
  \end{preprint}
  \begin{preprint}{Guba02}{Guba:2002b}
    \au{V.S.~Guba}
    \ti{On the Properties of the Cayley Graph of Richard Thompson's Group $F$}
    \lo{Preprint (2002), arXiv:math.GR/0211396 v1}{}
  \end{preprint}
  \begin{book}{GuSa97}{Guba.Sapir:1997}
    \au{V.S.~Guba, M.S.~Sapir}
    \ti{Diagram Groups}
    \lo{Mem. Amer. Math. Soc. 130 (1997)}{}
  \end{book}
  \begin{article}{GuSa99}{Guba.Sapir:1999}
    \au{V.S.~Guba, M.V.~Sapir}
    \ti{On subgroups of the R. Thompson group $F$ and other diagram groups}
    \lo{Math. USSR Sbornik 190 (1999), no. 7-8}{1077--1130}
   \end{article}
  \begin{article}{Hare85}{Harer:1985}
    \au{J.L.~Harer}
    \ti{Stability of the homology of the mapping class groups of orientable surfaces}
    \lo{Annals of Mathematics 121 (1985)}{215 -- 249}
  \end{article}
  \begin{article}{Hare86}{Harer:1986}
    \au{J.L.~Harer}
    \ti{The virtual cohomological dimension of the mapping class group of an orientable surface.}
    \lo{Inventiones mathematicae 84 (1986)}{157 -- 176}
  \end{article}
  \begin{article}{Harv79}{Harvey:1979}
    \au{W.J.~Harvey}
    \ti{Geometric structure of surface mapping class groups}
    \lo{In \cite{Wall:1979}}{255 -- 269}
  \end{article}
  \begin{article}{HaMe96}{Harlander.Meinert:1996}
    \au{J.~Harlander, H.~Meinert}
    \ti{Higher generation subgroup sets and the virtual cohomological dimension of graph
      products of finite groups}
    \lo{Journal of the London Mathematical Society 53 (1996)}{99 -- 117}
  \end{article}
  \begin{book}{Harp00}{Harpe:2000}
    \au{P.~de~la~Harpe}
    \ti{Topics in Geometric Group Theory}
    \lo{University of Chicago Press (2000)}{}
  \end{book}
  \begin{book}{Hat01}{Hatcher:2001}
    \au{A.~Hatcher}
    \ti{Algebraic Topology}
    \lo{Cambridge University Press (2001)}{}
    \www{http://www.math.cornell.edu/\~{}hatcher/AT/ATpage.html}
  \end{book}
  \begin{article}{HaVo96}{Hatcher.Vogtmann:1996}
    \au{A.~Hatcher, K.~Vogtmann}
    \ti{Isoperimetric Inequalities for Automorphism Groups of Free Groups}
    \lo{Pacific Journal of Mathematics 173 (1996)}{425 -- 441}
  \end{article}
  \begin{preprint}{Heyd99}{Heydebreck:1999}
    \au{A.~von~Heydebreck}
    \ti{Homotopy properties of certain complexes associated to spherical buildings}
    \lo{Preprint, (Frankfurt 1999)}{}
  \end{preprint}
  \begin{report}{Higm74}{Higman:1974}
    \au{G.~Higman}
    \ti{Finitely Presented Infinite Simple Groups}
    \lo{Australian Nat.\ University, Notes in Pure Mathematics 8 (Canberra, 1974)}{}
  \end{report}
  \begin{article}{Hows54}{Howson:1954}
    \au{A.G.~Howson}
    \ti{On the intersection of finitely generated free groups}
    \lo{Journal of the London Mathematical Society 29 (1954)}{428 -- 434}
  \end{article}
  \begin{article}{Inci97}{Incitti:1997}
    \au{R.~Incitti}
    \ti{Regularities on the Cayley Graphs of Groups of Linear Growth}
    \lo{European Journal of Combinatorics 18 (1997)}{175 -- 178}
  \end{article}
  \begin{article}{Ivan97}{Ivanov:1997}
    \au{N.V.~Ivanov}
    \ti{Automorphisms of complexes of curves and of Teichm^^fcller spaces}
    \lo{International Mathematical Research Notices (1997) no. 14}{651 - 666}
  \end{article}
  \begin{article}{John83}{Johnson:1983}
    \au{D.~Johnson}
    \ti{The structure of the Torelli group I: A finite set of generators for $\mathcal{J}$}
    \lo{Annals of Mathematics 118 (1983)}{423 -- 442}
  \end{article}
  \begin{article}{Kapo02}{Kapovich:2002}
    \au{I.~Kapovich}
    \ti{A note on the Po\'{e}naru condition}
    \lo{Journal of Group Theory 5 (2002)}{119 -- 127}
  \end{article}
  \begin{manuscript}{Kirb95}{Kirby:1995}
    \au{R.~Kirby}
    \ti{Problems in Low-Dimensional Topology}
    \lo{Manuskript (Berkeley, 1995)}{}
    \www{http://www.math.berkeley.edu/\~{}kirby/}
  \end{manuscript}
  \begin{article}{KM98a}{Kharlampovic.Myasnikov:1998a}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Tarski's problem about the elementary theory of free groups has a positive
      solution}
    \lo{ERA-AMS (1998)}{101 -- 108}
  \end{article}
  \begin{article}{KM98b}{Kharlampovic.Myasnikov:1998b}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Irreducible affine varieties over a free group. I: Irreducibility of quadratic
      equations and Nullstellensatz} % (paper 1 on the theory of a free group)
    \lo{Journal of Algebra 200 (1998)}{472 -- 516}
  \end{article}
  \begin{article}{KM98c}{Kharlampovic.Myasnikov:1998c}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Irreducible affine varieties over a free group. II: Systems in row-echelon form
      and description of residually free groups} % (paper 2 on the theory of a free group)
    \lo{Journal of Algebra 200,(1998)}{517 -- 570}
  \end{article}
  \begin{article}{KM00a}{Kharlampovic.Myasnikov:2000a}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Implicit function theorem over free groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{KM00b}{Kharlampovic.Myasnikov:2000b}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Equations over fully residually free groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{KM00c}{Kharlampovic.Myasnikov:2000c}
    \au{O.~Kharlampovic, A.~Myasnikov}
    \ti{Elementary theory of free nonabelian groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Knes64}{Kneser:1964}%
    \au{M.~Kneser}
    \ti{{\selectlanguage{german}Erzeugende und Relationen verallgemeinerter Einheitengruppen}}
    \lo{{\selectlanguage{german}Journal f\"u{}r die Reine und Angewandte Mathematik} 214/215 (1964)}{345 -- 349}
  \end{article}
  \begin{thesis}{Koch97}{Kochloukova:1997}
    \au{D.~Kochloukova}
    \ti{The FP${}^m$-Conjecture for a class of metabelian groups}
    \lo{PhD thesis (Cambridge, 1997)}{}
  \end{thesis}
  \begin{thesis}{Kram95}{Krammer:1995}
    \au{D.~Krammer}
    \ti{The conjugacy problem for Coxeter groups}
    \lo{PhD thesis (Utrecht 1995)}{}
  \end{thesis}
  \begin{article}{KMcC97}{Kristic.McCool:1997}
    \au{S.~Kristi\'{c}, J.~McCool}
    \ti{The non-finite presentability of $IA(F_3)$ and $\GL_2(\mathrm{Z}[t,t^{-1}])$}
    \lo{Inventiones mathematicae 129 (1997)}{595 -- 606}
  \end{article}
  \begin{book}{LSch77}{Lyndon.Schupp:1977}
    \au{R.C.~Lyndon, P.E.~Schupp}
    \ti{Combinatorial Group Theory}
    \lo{{\selectlanguage{german}Ergebnisse der Mathematik und ihrer Grenzgebiete 89} (Springer, 1977)}{}
  \end{book}
  \begin{article}{Lys85}{Lysenok:1985}
    \au{I.G.~Lysenok}
    \ti{A System of Defining Relations for a Grigorchuk Group}
    \lo{Translations: Matematicheskie Zametki 38 (1985)}{784 -- 792}
  \end{article}
  \begin{article}{Macb64}{Macbeath:1964}%
    \au{A.M.~Macbeath}
    \ti{Groups of homeomorphisms of a simply connected space}
    \lo{Annals of Math 79 (1964)}{473--488}
  \end{article}
  \begin{article}{Magn34}{Magnus:1934}
    \au{W.~Magnus}
    \ti{{\selectlanguage{german}^^dcber $n$-dimensionale Gittertransformationen}}
    \lo{Acta mathematica 64 (1934)}{353 -- 367}
  \end{article}
  \begin{book}{Magn74}{Magnus:1974}
    \au{W.~Magnus}
    \ti{Noneuclidean Tesselations and their Groups}
    \lo{Academic Press (New York, London 1974)}{}
  \end{book}
  \begin{article}{Maka82}{Makanin:1982}
    \au{G.S.~Makanin}
    \ti{Equations in a Free Group}
    \lo{Math. USSR Izvestiya 21 (1983)}{483 -- 546}
  \end{article}
  \begin{article}{McCM86}{McCullough.Miller:1986}
    \au{D.~McCullough, A.~Miller}
    \ti{The genus $2$ Torelli group is not finitely generated}
    \lo{Topology Applications 22 (1986) no.\ 1}{43 -- 49}
  \end{article}
  \begin{article}{Mess92}{Mess:1992}
    \au{G.~Mess}
    \ti{The Torelli groups for genus $2$ and $3$ surfaces}
    \lo{Topology 31 (1992) no. 4}{775 -- 790}
  \end{article}
  \begin{article}{Meie82}{Meier:1982}
    \au{D.~Meier}
    \ti{Non-Hopfian Groups}
    \lo{Journal of the London Mathematical Society 26 (1982)}{265 -- 270}
  \end{article}
  \begin{article}{MMV98}{Meier.Meinert.VanWyk:1998}
    \au{J.~Meier, H.~Meinert, L.~VanWyk}
    \ti{Higher generation subgroup sets and the $\Sigma$-invariants of graph groups}
    \lo{Commentarii Mathematici Helvetici 73 (1998)}{22 -- 44}
  \end{article}
  \begin{article}{Mein96}{Meinert:1996}%
    \au{H.~Meinert}
    \ti{The homological invariants for metabelian groups of
        finite Pr\"u{}fer rank: a proof of the $\Sigma^m$-conjecture}
    \lo{Proceedings of the London Mathematical Society 72 (1996)}{385 -- 424}
  \end{article}
  \begin{article}{Mein97}{Meinert:1997}%
    \au{H.~Meinert}
    \ti{Actions on $2$-complexes and the homotopical invariant
        $\Sigma^2$ of a group}
    \lo{Journal of Pure and Applied Algebra 119 (1997)}{297 -- 317}
  \end{article}
  \begin{thesis}{Mein93}{Meinert:1993}%
    \au{H.~Meinert}
    \ti{{\selectlanguage{german}Die h\"o{}heren geometrischen Invarianten~$\Sigma^m$ von Gruppen
        via Operationen auf CW-Komplexen und der Beweis der
        $\Sigma^m$-Vermutung f\"u{}r metabelsche Gruppen endlichen
        Pr\"u{}fer-Ranges}}
    \lo{PhD thesis (Frankfurt, 1993)}{}
  \end{thesis}
  \begin{article}{MiSh98}{Miller.Shapiro:1998}
    \au{C.F.~Miller~III, M.~Shapiro}
    \ti{Solvable Baumslag-Solitar Groups are not Almost Convex}
    \lo{Geometria Dedicata 72 (1998)}{123 -- 127}
  \end{article}
  \begin{book}{Mois77}{Moise:1977}
    \au{E.E.~Moise}
    \ti{Geometric Topology in Dimensions 2 and 3}
    \lo{Springer GTM 47}{}
  \end{book}
  \begin{article}{Neum37}{Neumann:1937}%
    \au{B.H.~Neumann}
    \ti{Some remarks on infinite groups}
    \lo{Journal of the London Mathematical Society 12 (1937)}{120 -- 127}
  \end{article}
  \begin{article}{Neum55}{Neumann:1955}
    \ti{On the intersection of finitely generated free groups}
    \au{H.~Neumann}
    \lo{Publ. Math. Debrecen 4 (1955-56)}{186 -- 189}
    [\lo{Addendum: ibid. 5 (1957-58)}{128}]
  \end{article}
  \begin{article}{Nosk97}{Noskov:1997}
    \au{G.A.~Noskov}
    \ti{The Bieri-Strebel invariant and homological finiteness conditions for metabelian groups}
    \lo{Algebra and Logic 36 (1997)}{117 -- 132}
  \end{article}
  \begin{book}{O'Me73}{OMeara:1973}%
    \au{O.T.~O'Meara}
    \ti{Introduction to Quadratic Forms}
    \lo{Berlin, Heidelberg, New~York (Springer, 1973)}{}
  \end{book}
  \begin{thesis}{Prov77}{Provan:1977}
    \au{J.S.~Provan}
    \ti{Decopositions, shellings and diameters of simplicial complexes and convex polytopes}
    \lo{Thesis, Cornell University (1977)}{}
  \end{thesis}
  \begin{article}{Quil78}{Quillen:1978}
    \au{D.~Quillen}
    \ti{Homotopy Properties of the Poset of Nontrivial $p$-Subgroups of a Group}
    \lo{Advances in Mathematics 28 (1978)}{101 -- 128}
  \end{article}
  \begin{article}{Ragh68}{Raghunatan:1968}
    \au{M.S.~Raghunatan}
    \ti{A Note on Quotients of Real Algebraic Groups by Arithmetic Subgroups}
    \lo{Inventiones mathematicae 4 (1968)}{318 -- 335}
  \end{article}
  \begin{article}{Razb84}{Razborov:1984}
    \au{A.A.~Razborov}
    \ti{On Systems of Equations in a Free Group}
    \lo{Math. USSR Izvestiya 25 (1985)}{115 -- 162}
  \end{article}
  \begin{thesis}{Renz88}{Renz:1988}
    \au{B.~Renz}
    \ti{{\selectlanguage{german}Geometrische Invarianten und Endlichkeitseigenschaften von
        Gruppen}}
    \lo{PhD thesis (Frankfurt, 1988)}{}
  \end{thesis}
  \begin{preprint}{Rile02}{Riley:2002}
    \au{T.R.~Riley}
    \ti{The geometry of groups satisfying weak almost-convexity or weak geodesic-combability conditions}
    \lo{Journal of Group Theory 5 (2002)}{513 -- 525}
  \end{preprint}
  \begin{book}{Rona89}{Ronan:1989}%
    \au{M.~Ronan}
    \ti{Lectures on Buildings}
    \lo{Perspectives in Mathematics,
        Academic Press, San~Diego, London (1989)}{}
  \end{book}
  \begin{article}{SBR02}{Birget.Sapir.Rips:2002}
    \au{M.V.~Sapir, J.C.~Birget, E.~Rips}
    \ti{Isoperimetric and Isodiametric Functions of Groups}
    \lo{Annals of Mathematics 156 (2002)}{345 -- 466}
  \end{article}
  \begin{article}{Salv94}{Salvetti:1994}
    \au{M.~Salvetti}
    \ti{The Homotopy Type of Artin Groups}
    \lo{Mathematical Research Letters 1 (1994)}{565 -- 577}
  \end{article}
  \begin{article}{Se01a}{Sela:2001a}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups I: Makanin-Razborov diagrams}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01b}{Sela:2001b}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups  II: Completions, closures and formal solutions}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01c}{Sela:2001c}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups III: Rigid and solid solutions}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01d}{Sela:2001d}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups IV: An iterative procedure for validation of a sentence}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01e}{Sela:2001e}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups  V: Quantifier elimination}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01f}{Sela:2001f}%
    \au{Z.~Sela}
    \ti{Diphantine Geometry over Groups VI: The elementary theory of a free group}
    \lo{preprint}{}
  \end{article}
  \begin{book}{Serr77}{Serre:1977}%
    \au{J.-P.~Serre}
    \ti{{\selectlanguage{french}Arbres, amalgames, $SL_2$}}
    \lo{Asterique 46 (1977)}{}
  \end{book}
  \begin{article}{Serr79}{Serre:1979}
    \au{J.P.~Serre}
    \ti{Arithmetic Groups}
    \lo{In \cite{Wall:1979}}{105 -- 136}
  \end{article}
  \begin{article}{ShSt95}{Shapiro.Stein:1995}
    \au{M.~Shapiro, M.I.~Stein}
    \ti{Almost Convex Groups and the Eight Geometries}
    \lo{Geometria Dedicata 55 (1995)}{125 -- 140}
  \end{article}
  \begin{article}{Shor90}{Short:1990}
    \au{H.~Short}
    \ti{Quasiconvexity and a Theorem of Howson}
    \lo{in \cite{Ghys.Haefliger.Verjovsky:1990}}{168 -- 176}
  \end{article}
  \begin{preprint}{Skor??}{Skora:unknown}
    \au{R.~Skora}
    \ti{Deformation of Length Functions in Groups}
    \lo{Preprint (????)}{}
  \end{preprint}
  \begin{article}{Smal57}{Smale:1957}
    \au{S.~Smale}
    \ti{A Vietoris Mapping Theorem for Homotopy}
    \lo{Proceedings of the American Mathematical Society 8 (1957)}{604 -- 610}
  \end{article}
  \begin{article}{SV87a}{Smillie.Vogtmann:1987a}
    \au{J.~Smillie, K.~Vogtmann}
    \ti{A Generating Function for the Euler Characteristic of Out$(F_n)$}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{329 -- 348}
  \end{article}
  \begin{article}{SV87b}{Smillie.Vogtmann:1987b}
    \au{J.~Smillie, K.~Vogtmann}
    \ti{Automorphisms of Graphs, $p$-subgroups of Out$(F_n)$ and the Euler Characteristic of Out$(F_n)$}
    \lo{Journal of Pure and Applied Algebra 49 (1987)}{182 -- 200}
  \end{article}
  \begin{book}{Span66}{Spanier:1966}
    \au{E.H.~Spanier}
    \ti{Algebraic Topology}
    \lo{Springer, New York (1966)}{}
  \end{book}
  \begin{article}{Stal68}{Stallings:1968}
    \au{J.R.~Stallings}
    \ti{On torsion-free groups with infinitely many ends}
    \lo{Annals of Mathematics 88 (1968)}{312 -- 334}
  \end{article}
  \begin{article}{Stal88}{Stallings:1988}
    \au{J.~Stallings}
    \ti{Foldings of $G$-trees}
    \lo{in \cite{Alperin:1991}}{355 -- 368}
  \end{article}
  \begin{notes}{Stei68}{Steinberg:1968}%
    \au{R.~Steinberg}
    \ti{Lectures on Chevalley Groups,
        Notes prepared by John Faulkner and Robert Wilson.}
    \lo{Yale University, New Haven, Connecticut, (1968)}{}
  \end{notes}
  \begin{article}{Stre84}{Strebel:1984}%
    \au{R.~Strebel}
    \ti{Finitely Presented Solvable Groups}
    \lo{In \cite{Gruenberg.Roseblade:1984}}{257 -- 314}
  \end{article}
  \begin{article}{Stuh76}{Stuhler:1976}%
    \au{U.~Stuhler}
    \ti{{\selectlanguage{german}Zur Frage der endlichen Pr\"a{}sentiertheit gewisser
        arithmetischer Gruppen im Funktionenk\"o{}rperfall}}
    \lo{{\selectlanguage{german}Mathematische Annalen 224 (1976)}}{217 -- 232}
  \end{article}
  \begin{article}{Stuh80}{Stuhler:1980}%
    \au{U.~Stuhler}
    \ti{Homological properties of certain arithmetic groups in
        the function field case}
    \lo{Inventiones mathatematicae 57 (1980)}{263 -- 281}
  \end{article}
  \begin{article}{Symo98}{Symonds:1998}%
    \au{P.~Symonds}
    \ti{The orbit space of the $p$-subgroup complex is contractible}
    \lo{Commentarii Mathematici Helvetici 73 (1998)}{400 -- 405}
  \end{article}
  \begin{thesis}{Tiem94}{Tiemeyer:1994}%
    \au{A.~Tiemeyer}
    \ti{{\selectlanguage{german}Kompaktheitseigenschaften lokalkompakter Gruppen}}
    \lo{PhD thesis (Bielefeld, 1994)}{}
  \end{thesis}
  \begin{article}{Tiem97}{Tiemeyer:1997}%
    \au{A.~Tiemeyer}
    \ti{A Local-Global Principle for Finiteness Properties of
      $S$-Artihmetic Groups over Number Fields}
    \lo{Transformation Groups 2 (1997)}{215 -- 223}
%    (confere~\cite{Abels.Tiemeyer:1997})
  \end{article}
  \begin{article}{Tits72}{Tits:1972}%
    \au{J.~Tits}
    \ti{Free Subgroups in Linear Groups}
    \lo{Journal of Algebra 20 (1972)}{250 -- 270}
  \end{article}
  \begin{article}{Tits87}{Tits:1987}%
    \au{J.~Tits}
    \ti{Uniqueness and Presentations of Kac-Moody Groups over Fields}
    \lo{Journal of Algebra~105 (1987)}{542 -- 573}
  \end{article}
  \begin{article}{Vogt90}{Vogtmann:1990}
    \au{K.~Vogtmann}
    \ti{Local Structure of some $\mathop{\mathrm{OUT}}(F_n)$-Complexes}
    \lo{Proceedings of the Edinburgh Mathematical Society (1990)}{367 -- 379}
  \end{article}
  \begin{preprint}{Vogt00}{Vogtmann:2000}
    \au{K.~Vogtmann}
    \ti{Automorphisms of Free Groups and Outer Space}
    \lo{To appear in the special issue of Geometriae Dedicata for the June, 2000 Haifa Conference
        on Geometric Group Theory}{}
  \end{preprint}
  \begin{article}{Wall65}{Wall:1965}
    \au{C.T.C.~Wall}
    \ti{Finiteness Conditions for CW-Complexes}
    \lo{Annals of Mathematics 81 (1965)}{56 -- 69}
  \end{article}
  \begin{book}{Wall79}{Wall:1979}
    \ed{C.T.C.~Wall}
    \ti{Homological Group Theory}
    \lo{LMS Lecture Notes 35, Cambridge University Press (Cambridge 1979)}{}
  \end{book}
  \begin{book}{Weil73}{Weil:1973}%
    \au{A.~Weil}
    \ti{Basic Number Theory}
    \edition{Reprint of the Second Edition (1973)}
    \lo{Springer Classics in Mathematics, Berlin Heidelberg (1995)}{}
  \end{book}
  \begin{book}{Whit92}{White:1992}
    \ed{N.~White}
    \ti{Matroid Applications, volume 40 of Encyclopedia of Mathematics}
    \lo{Cambridge University Press (1992)}{}
  \end{book}
\end{references}
\endinput


==> notation.tex <==
\ProvidesFile{notation.tex}[2000/10/05 KUB]

% \newcommand{\LabelTop}{\mathrm{top}}
% \newcommand{\LabelBot}{\mathrm{bot}}
% 
\renewcommand{\setminus}{-}
% 
\newcommand{\PositiveReals}{\RRR^+}
% 
% \newcommand{\Choose}[2]{\left(\begin{array}{@{}c@{}}#1\\#2\end{array}\right)}
% 
% \newcommand{\SquareOf}[1]{\ToThePower{#1}{\Two}}
% 
% %
% % Generalities
% %
% 
% \newvariable{\TheVariable}{x}
% \newvariable{\AltVariable}{y}
% 
% \newcommand{\FloorOf}[1]{\left\lfloor#1\right\rfloor}
% \newcommand{\CeilingOf}[1]{\left\lceil#1\right\rceil}
% 
% \newcommand{\CycleOf}[1]{\left[#1\right]}
% 
% \newcommand{\ComplementOf}[1]{#1^{\mathrm{c}}}
\newcommand{\FactorialOf}[1]{#1!}
% \newcommand{\ChooseFrom}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
% 
% \newcommand{\DualOf}[1]{#1^{*}}
% 
% %
% % Elementary Functions
% %
% \newcommand{\LbOf}{\log_2\EvalAt}
% 
% %
% % Out F_n
% %
% \newvariable{\TheAutomorphism}{\alpha}
% \newvariable{\AltAutomorphism}{\beta}
% \newvariable{\TheOutomorphism}{\overline\TheAutomorphism}
% \newvariable{\AltOutomorphism}{\overline\AltAutomorphism}
% \newvariable{\InnerAutomorphism}{\iota}
% \newvariable{\Korelli}{K}
% \newvariable{\OutKorelli}{\bar{\Korelli}}
% \newvariable{\Torelli}{T}
% \newvariable{\TheJohnsonHomomorphism}{\Phi}
% \newvariable{\TheKohnsonHomomorphism}{\Phi}
% \newvariable{\TheMagnusGenerator}{K}
\newvariable{\TheGraph}{\Gamma}
% \newvariable{\TheSubgraph}{\Delta}
% \newvariable{\AltGraph}{\Delta}
% \newvariable{\TheLabeling}{\rho}
% \newvariable{\AltLabeling}{\tau}
% \newvariable{\Rose}{\Rho}
% \newcommand{\FreeAbelian}[1][]{\ZZZ\OptExponent[#1]}
\newcommand{\LinkOf}[2][]{\Lk\IfNonEmpty{#1}{_{#1}}\negthinspace\left(#2\right)}
\newcommand{\StarOf}[2][]{\St\IfNonEmpty{#1}{_{#1}}\negthinspace\left(#2\right)}
\newcommand{\Lk}{\mathop{\mathrm{Lk}}\nolimits}
\newcommand{\St}{\mathop{\mathrm{St}}\nolimits}
\newcommand{\compose}{\circ}
\newcommand{\AbsValueOf}[1]{\left|#1\right|}
% \newcommand{\NormOf}{\AbsValueOf}
\newcommand{\CardOf}{\AbsValueOf}
% \newcommand{\EilenbergMaclane}[1][\TheGroup]{\mathrm{K}\left(#1,\One\right)}
% \newcommand{\GroupRing}[2][\ZZZ]{#1#2}
\newvariable{\HomotopyGroup}{\pi}
\newcommand{\HomotopyOf}[2][*]{\HomotopyGroup[#1]\negthinspace\left(#2\right)}
% \newvariable{\HomologyGroup}{\H}
% \newcommand{\HomologyOf}[1][*]{\HomologyGroup[#1]\OptExponentParentheses}
% \newcommand{\FundamentalGroup}[1][1]{\pi_{#1}}
% \newcommand{\FundamentalGroupOf}[2][]{%
%   \IfEmptyThenElse{#1}{%
%     \HomotopyGroup_{1}\EvalAt{#2}%
%   }{%
%     \HomotopyGroup_{1}\EvalAt{#2,#1}%
%   }
% }
% \newvariable{\FundamentalGroupTransformation}{\Phi}
% \newvariable{\ReducedHomologyGroup}{\tilde{\HomologyGroup}}
% \newcommand{\ReducedHomologyOf}[1][*]{\ReducedHomologyGroup[#1]\OptExponentParentheses}
% \newcommand{\CohomologyOf}[1][*]{\HomologyGroup\IfNonEmpty{#1}{^{#1}}\OptIndexParentheses}
% \newcommand{\CircularHomologyOf}[1][*]{\overline{\HomologyGroup}\IfNonEmpty{#1}{_{#1}}\OptExponentParentheses}
% \newcommand{\HomeoOf}{\operatorname{Homeo}\EvalAt}
% \newcommand{\PermOf}{\operatorname{Perm}\EvalAt}
% \newcommand{\TheDegree}{d}
% \newcommand{\Maps}{\operatorname{Map}\OptIndexParentheses}
% \newcommand{\MapsFromTo}[2]{\operatorname{Map}\EvalAt{{#1},{#2}}}
% 
% \newvariable{\homotopic}{\sim}
% 
% 
% %
% % Stallings Folds
% %
% \newvariable{\TheStFold}{f}
% \newvariable{\TheGraphMorphism}{\varphi}
% \newvariable{\AltGraphMorphism}{\psi}
% 
% %
% %
% %
% 
% \newcommand{\RankOf}{\operatorname{rk}\EvalAt}
\newcommand{\crossprod}{\times}
% \newcommand{\directsum}{\oplus}
% 
\newvariable{\TheNumber}{n}
% \newvariable{\AltNumber}{m}
% \newvariable{\TheSize}{r}
% \newvariable{\TheBigNumber}{N}
% \newvariable{\AltBigNumber}{M}
% \newvariable{\TheBigReal}{L}
% 
% \newvariable{\OuterSpace}{\mathcal{X}}
% \newvariable{\AuterSpace}{\mathcal{Y}}
% 
% \newvariable{\TheCoin}{C}
% \newvariable{\TheProbability}{p}
% \renewcommand{\TheProbabilityOf}{P\OptIndexParentheses}
% 
% %
% % Combinatorics
% %
% \newcommand{\StirlingSec}[2]{S\EvalAt{#1,#2}}
% \newvariable{\TheDerangements}{d}
% \newvariable{\ThePermutation}{\pi}
% 
% %
% % Finiteness Properties
% %
\newcommand{\FType}[1][]{\ensuremath{\mathrm{F}\IfNonEmpty{#1}{_{#1}}}}
\newcommand{\FPType}[1][]{\ensuremath{\mathrm{FP}\IfNonEmpty{#1}{_{#1}}}}
% \newvariable{\TheFType}{m}
% \newvariable{\TheFPType}{\TheFType}
% \newvariable{\TheGroupComplex}{Y}
% \newvariable{\TheInteger}{s}
% \newvariable{\AltInteger}{t}
% \newvariable{\TheGeneration}{s}
% \newvariable{\AltGeneration}{t}
% \newvariable{\LastIndex}{n}
% \newvariable{\TheLastIndex}{r}
% \newvariable{\AltLastIndex}{s}
% 
% \newvariable{\TheWhole}{n}
% \newvariable{\AltWhole}{m}
% \newvariable{\TheBigWhole}{N}
% \newvariable{\AltBigWhole}{M}
% \newvariable{\ThePlayer}{A}
% \newvariable{\AltPlayer}{B}
% \newvariable{\TheEvie}{E}
% \newvariable{\TheDodie}{D}
% 
\newcommand{\DimOf}[2][]{\dim\IfNonEmpty{#1}{_{#1}}\EvalAt{#2}}
% 
% \newcommand{\Homs}{\Hom\EvalAt}
% 
% %
% \newvariable{\TheProjModule}{P}
% %
% \newvariable{\TheGeoDim}{d}%_g}
% \newvariable{\TheCohomDim}{d}%_c}
% %
% %
% \newvariable{\TheBotLevel}{\One}
% \newvariable{\TheSecLevel}{\Two}
% \newvariable{\TheTopLevel}{n}
% %\newvariable{\TheRank}{\TheTopLevel}
% \newcommand{\OppIt}[1]{-#1}%{\overline{#1}}
% \newvariable{\InvBotLevel}{\OppIt{\TheBotLevel}}
% \newvariable{\InvSecLevel}{\OppIt{\TheSecLevel}}
% \newvariable{\InvTopLevel}{\OppIt{\TheTopLevel}}
% \newvariable{\LevelSet}{L}
% \newcommand{\lowerthan}{<}
% \newvariable{\LabelSet}{M}
% \newvariable{\TheLabel}{m}
% \newvariable{\OppLabel}{\OppIt{\TheLabel}}
% \newvariable{\TheLevel}{s}
% \newvariable{\AltLevel}{t}
% \newvariable{\Partitions}{P}
% \newvariable{\ThePartition}{p}
% \newvariable{\AltPartition}{q}
% \newcommand{\PosPartOf}[1]{#1[+]}
% \newcommand{\NegPartOf}[1]{#1[-]}
% 
% \newvariable{\Metric}{\mu}
% 
% \newvariable{\LinkModel}{X}
% \newvariable{\DescModel}{X^-}
% 
% \newvariable{\HomologyClass}{v}
% \newexpvector{\Coordinate}{v}
% \newcommand{\TwoIndexHomologyClass}[2]{v_{#1}^{(#2)}}
% 
% \newMap{\SplitSetOf}{s}
% \newMap{\PosSplitSetOf}{s_+}
% \newMap{\BottomLabelOf}{\mathrm{bot}}
% \newMap{\SignatureOf}{\sign}
% 
% \newvariable{\LinkZero}{\LinkModel_0}
% \newvariable{\LinkOne}{\LinkModel_1}
% \newvariable{\LinkHalf}{\LinkModel_{\OneHalf}}
% \newmap{\BotDistance}{d_{\Bot}}
% \newmap{\LinkOneToCube}{\pi}
% \newindexedmap{\LabelDist}{\lambda}
% \newmap{\AbsValOfAffineMap}{\phi}
% 
% %{\frac{#1}{\AbsValueOf{#1}}}
% \newMapTwo{\RelHeightOf}{h}
\newMap{\HeightOf}{h}
% \newconst{\ZeroSequence}{\underbar{0}}
% 
% \newvariable{\TheInt}{k}
% \newvariable{\AltInt}{l}
% 
\newvariable{\TheIndex}{i}
\newvariable{\AltIndex}{j}
% \newvariable{\ThirdIndex}{k}
% \newvariable{\ForthIndex}{l}
% \newvariable{\FourthIndex}{l}
% \newvariable{\TheBigIndex}{m}
% \newvariable{\AltBigIndex}{n}
% 
% \newvariable{\TheMultiIndex}{I}
% \newvariable{\AltMultiIndex}{J}
% 
% 
% \newvariable{\TheExponent}{k}
% \newvariable{\AltExponent}{l}
% 
% \iffalse
%   \newcommand{\Top}{\Three}
%   \newcommand{\Med}{\Two}
%   \newcommand{\Bot}{\One}
%   \newcommand{\TOP}{\OppIt{\Top}}
%   \newcommand{\MED}{\OppIt{\Med}}
%   \newcommand{\BOT}{\OppIt{\Bot}}
% \fi
%   
% \makeatletter
%   \newcommand{\LetterToLabel}[1]{%
%     \begingroup
%       \def\tempa{#1}
%       \def\b{b}
%       \def\B{B}
%       \def\m{m}
%       \def\M{M}
%       \def\t{t}
%       \def\T{T}
%       \def\next{\relax}
%       \ifx\tempa\b
%         \def\next{\Bot}
%       \fi
%       \ifx\tempa\B
%         \def\next{\BOT}
%       \fi
%       \ifx\tempa\m
%         \def\next{\Med}
%       \fi
%       \ifx\tempa\M
%         \def\next{\MED}
%       \fi
%       \ifx\tempa\t
%         \def\next{\Top}
%       \fi
%       \ifx\tempa\T
%         \def\next{\TOP}
%       \fi
%     \expandafter\endgroup\next
%   }
%   \newcommand{\LetterToLevel}[1]{%
%     \begingroup
%       \def\tempa{#1}
%       \def\b{b}
%       \def\B{B}
%       \def\m{m}
%       \def\M{M}
%       \def\t{t}
%       \def\T{T}
%       \def\next{\relax}
%       \ifx\tempa\b
%         \def\next{\Bot}
%       \fi
%       \ifx\tempa\B
%         \def\next{\Bot}
%       \fi
%       \ifx\tempa\m
%         \def\next{\Med}
%       \fi
%       \ifx\tempa\M
%         \def\next{\Med}
%       \fi
%       \ifx\tempa\t
%         \def\next{\Top}
%       \fi
%       \ifx\tempa\T
%         \def\next{\Top}
%       \fi
%     \expandafter\endgroup\next
%   }
%   \newcommand{\LetterToSign}[1]{%
%     \begingroup
%       \def\tempa{#1}
%       \def\b{b}
%       \def\B{B}
%       \def\m{m}
%       \def\M{M}
%       \def\t{t}
%       \def\T{T}
%       \def\next{\relax}
%       \ifx\tempa\b
%         \def\next{+}
%       \fi
%       \ifx\tempa\B
%         \def\next{-}
%       \fi
%       \ifx\tempa\m
%         \def\next{+}
%       \fi
%       \ifx\tempa\M
%         \def\next{-}
%       \fi
%       \ifx\tempa\t
%         \def\next{+}
%       \fi
%       \ifx\tempa\T
%         \def\next{-}
%       \fi
%     \expandafter\endgroup\next
%   }
%   \def\LetterList#1#2{%
%     \begingroup
%       \def\tempa{#2}
%       \def\End{\end}
%       \ifx\tempa\End
%         \def\next{\LetterToLabel#1}
%       \else
%         \def\next{\LetterToLabel#1, \LetterList#2}
%       \fi
%     \expandafter\endgroup\next
%   }
%   \def\LetterSum#1#2{%
%     \begingroup
%       \def\tempa{#2}
%       \def\End{\end}
%       \ifx\tempa\End
%         \ifprintsign
%           \def\next{\LetterToSign#1\Coordinate[{\LetterToLevel#1}]}
%         \else
%           \def\next{\Coordinate[{\LetterToLevel#1}]}
%         \fi
%       \else
%         \ifprintsign
%           \def\next{\LetterToSign#1\Coordinate[{\LetterToLevel#1}]\LetterSum#2}
%         \else
%           \def\next{\Coordinate[{\LetterToLevel#1}]\LetterSum#2}
%         \fi
%       \fi
%     \expandafter\expandafter\expandafter\endgroup\expandafter\printsigntrue\next
%   }
%   
%   \newif\ifprintsign
%   
%   \renewcommand{\L}[1]{%
%     \left\{
%     \IfNonEmpty{#1}{%
%       \LetterList#1\end
%     }
%     \right\}
%   }
%   
%   \renewcommand{\S}[1]{%
%     \begingroup
%       \printsignfalse
%       \left|
%         \IfNonEmpty{#1}{%
%           \LetterSum#1\end
%         }
%       \right|
%     \endgroup
%   }
% 
%   
% \makeatother
% 
% \newvariable{\ThePresentation}{\mathcal{P}}
% \newvariable{\ThePresComplex}{K}
% \newvariable{\TheLinkComplex}{L}
% 
% \newvariable{\TheCatDiagram}{D}
% \newvariable{\TheMap}{f}
% \newvariable{\AltMap}{h}
% \newvariable{\TheMapCover}{\bar{\TheMap}}
% \newvariable{\TheGenerator}{x}
% \newvariable{\AltGenerator}{y}
% \newvariable{\FirstGenerator}{x}
% \newvariable{\SecondGenerator}{y}
% \newvariable{\ThirdGenerator}{z}
% \newvariable{\InvGenerator}{x^{-1}}
% \newvariable{\TheFreeGenerator}{x}
% \newvariable{\InvFreeGenerator}{x^{-1}}
% \newvariable{\FirstGen}{1}
% \newvariable{\LastGen}{m}
% \newvariable{\Relator}{R}
% \newvariable{\FirstRel}{1}
% \newvariable{\LastRel}{n}
\newvariable{\TheRank}{n}
% \newvariable{\TheFreeRank}{n}
% 
% \newvariable{\Word}{w}
% 
% %
% % Graphs
% %
\newvariable{\TheCompleteGraph}{K}
% \newvariable{\TheValency}{d}
% \newvariable{\TheRedValency}{\TheValency_{\mathrm{r}}}
% \newvariable{\TheBlueValency}{\TheValency_{\mathrm{b}}}
% \newvariable{\TheSetOfRedVertices}{\TheSetOfVertices_{\mathrm{r}}}
% \newvariable{\TheSetOfBlueVertices}{\TheSetOfVertices_{\mathrm{b}}}
% 
% \newcommand{\edgeof}{\in}
% \newcommand{\equivedge}{\sim\OptIndex}
% 
% \newvariable{\DerGraph}{\Gamma}
% \newvariable{\BlackGraph}{\DerGraph^{\mathrm{b}}}
% \newvariable{\RedGraph}{\DerGraph^{\mathrm{r}}}
% 
% \newcommand{\EdgeSymbol}{e}
% \newvariable{\LinkEdge}{\EdgeSymbol}
% \newvariable{\LinkEdgePos}{\EdgeSymbol^+}
% \newvariable{\LinkEdgeNeg}{\EdgeSymbol^-}
% 
% \newvariable{\SignSymbol}{\varepsilon}
% \newcommand{\LinkEdgeDir}[1][]{\EdgeSymbol^{\SignSymbol[#1]}\IfNonEmpty{#1}{_{#1}}}
% 
% \newcommand{\LinkEdgeInvDir}[1][]{\EdgeSymbol^{-\SignSymbol[#1]}\IfNonEmpty{#1}{_{#1}}}
% 
% \newvariable{\Index}{i}
% 
% \newmap{\Mirror}{\phi}
% 
% \newvariable{\FirstEdge}{1}
% \newvariable{\LastEdge}{r}
% 
% \newvariable{\WeightFunction}{W}
% \newvariable{\TotalWeight}{T}
% 
% \newcommand{\WeightOf}[2][]{%
%   \left\|
%     #2
%   \right\|_{#1}
% }
%   
% 
% \newvariable{\EdgePath}{P}
% \newvariable{\DerEdge}{\overrightarrow{\EdgeSymbol}}
% \newcommand{\EdgesSymbol}{\mathcal{E}}
% \newvariable{\TheEdgeSet}{\EdgesSymbol}
% \newMap{\EdgesOf}{\EdgesSymbol}
% \newcommand{\OrientedEdgesOf}{\TheOrientedEdgeSet\OptIndex}
% \newvariable{\TheOrientedEdgeSet}{\overrightarrow{\EdgesSymbol}}
\newcommand{\VerticesSymbol}{\mathcal{V}}
% \newcommand{\SimplicesSymbol}{\mathcal{S}}
\newvariable{\TheVertexSet}{\VerticesSymbol}
% \newvariable{\TheSimplexSet}{\SimplicesSymbol}
% \newvariable{\DerVertexSet}{\VerticesSymbol}
% \newcommand{\VerticesOf}[1]{\TheVertexSet[#1]}
% 
% \newvariable{\IncomingEdges}{I}
% 
% \newvariable{\TheBaseVertex}{\TheVertex_{\Zero}}
% 
% \newcommand{\SubdivAngleSymbol}{w}
% \newvariable{\MoldAngleSymbol}{d}
% \newvariable{\MoldAngle}{\MoldAngleSymbol}
% 
% \newvariable{\EulerChar}{\chi}
% \newvariable{\NumberOfEdges}{E}
% \newvariable{\NumberOfTwoCells}{F}
% \newvariable{\NumberOfVertices}{V}
% \newvariable{\TheCorner}{c}
% \newvariable{\AltCorner}{c'}
% \newvariable{\TheTwoCell}{f}
% \newvariable{\TheTwoComplex}{K}
% \newvariable{\TheSetOfVertices}{W}
% \newvariable{\AltSetOfVertices}{U}
\newvariable{\TheVertex}{v}
\newvariable{\AltVertex}{w}
% \newvariable{\ThirdVertex}{u}
% \newvariable{\TwoCellCurvatureCorners}{\kappa}
% \newvariable{\VertexCurvatureCorners}{\kappa}
% \newvariable{\TwoCellCurvatureEdges}{\bar\kappa}
% \newvariable{\VertexCurvatureEdges}{\bar\kappa}
% \newvariable{\WeightAt}{w}
% \newvariable{\EdgeToVertexWeight}{w^0}
% \newvariable{\EdgeToFaceWeight}{w^2}
% \newMap{\OrientedBoundaryOf}{\partial^+}
% \newindexedmap{\Boundary}{\partial}
\newMap{\BoundaryOf}{\partial}
\newvariable{\TheEdge}{e}
% \newvariable{\AltEdge}{\TheEdge_{\bullet}}
% \newvariable{\TheOrientedEdge}{\vec{\TheEdge}}% {\overrightarrow{\TheEdge}}
% \newvariable{\OppOrientedEdge}{\OppEdge{\TheOrientedEdge}}% {{\overleftarrow{\TheEdge}}
% \newvariable{\AltOrientedEdge}{\Vec{\TheEdge}_{\bullet}}% {\overrightarrow{\TheEdge}'}
% \newvariable{\AltOppOrientedEdge}{\OppEdge{\AltOrientedEdge}}% {\overleftarrow{\TheEdge}'}
% \newvariable{\OppEdge}{\mathrm{op}}
% \newcommand{\OppEdgeStar}[1]{{#1}^{\mathrm{op}}}
% \newvariable{\Orientation}{\mathrm{o}}
% \renewcommand{\OrientationOf}[1][]{\Orientation[#1]\EvalAt}
%   
% \newmap{\EdgeToVertexMap}{\mu}
% \newmap{\VertexToEdgeMap}{\lambda}
% \newmap{\VertexToInitialMap}{\lambda^\iota}
% \newmap{\VertexToTerminalMap}{\lambda^\tau}
% \newMap{\InitialVertexOf}{\iota}
% \newmap{\InitialVertex}{\iota}
% \newMap{\TerminalVertexOf}{\tau}
% \newmap{\TerminalVertex}{\tau}
% \newvariable{\TheInitialVertex}{i}
% \newvariable{\TheTerminalVertex}{t}
% \newvariable{\TheLinkVertex}{p}
% \newvariable{\TheRedEdge}{r}
% \newvariable{\TheBlackEdge}{b}
% \newvariable{\TipVertex}{\tilde{\TheTerminalVertex}}
% \newvariable{\TapVertex}{\tilde{\TheInitialVertex}}
% %\newvariable{\TheOrientedEdge}{\overrightarrow{\EdgeSymbol}}
% \newmap{\OrientedEdgeToRedEdgeMap}{R}
% \newmap{\OrientedEdgeToBlackEdgeMap}{B}
% 
% \newvariable{\TheMidPoint}{M}
% 
% %
% % Flows
% %
% \newvariable{\TheRealGroup}{\Lambda}
% \newindexedmap{\TheFlow}{\Phi}
% \newindexedmap{\TheSmallFlow}{\tilde{\TheFlow}}
% \newindexedmap{\TheNetProduction}{P}
% \newvariable{\TheCapacity}{C}
% \newcommand{\GraphBoundaryOf}{\partial}
% \newvariable{\TheSetOfEdges}{E}
% \newvariable{\TheSetOfOrientedEdges}{\TheOrientedEdgeSet_{\Zero}}
% \newvariable{\TheMinCutSet}{\TheOrientedEdgeSet[\mathrm{min}]}
% \newvariable{\TheComplementaryVertex}{v_{*}}
% \newvariable{\TheSink}{I}
% \newvariable{\TheSource}{O}
% \newvariable{\TheSattle}{A}
% 
% \newvariable{\MinTotalWeight}{\MoldAngleSymbol}
% \newvariable{\SubdivAngle}{\SubdivAngleSymbol}
% \newvariable{\StarSubdivAngle}{\SubdivAngleSymbol^*}
% 
% \newvariable{\AltCornerIndex}{k}
% \newvariable{\AltPosCorner}{c'}
% \newvariable{\CornerIndex}{i}
% \newvariable{\Corner}{c^\pm}
% \newcommand{\FirstCorner}{\Zero}
% \newcommand{\SecondCorner}{\One}
% \newcommand{\FirstOppCorner}{\FirstCorner}
% \newcommand{\FirstPosCorner}{\FirstCorner}
% \newcommand{\LastOppCorner}{\LastCorner}
% \newcommand{\LastPosCorner}{\LastCorner}
% \newcommand{\LastCorner}{\Two\TheRank}
% \newcommand{\NumberOfCorners}[0]{\Two\TheRank+1}
% \newvariable{\OppCorner}{c^-}
% \newvariable{\PosCorner}{c^+}
% \newvariable{\PosRedEdge}{r^+}
% \newvariable{\RedEdge}{r^\pm}
% \newvariable{\Successor}{\Corner'}
% \newvariable{\TheCornerIndex}{i}
% \newvariable{\ThePosCorner}{c}
% \newvariable{\ThirdCornerIndex}{j}
% 
% \newvariable{\PosSattle}{a^+}
% \newvariable{\PosSource}{o^+}
% \newvariable{\PosSink}{i^+}
% \newvariable{\OppSattle}{a^-}
% \newvariable{\OppSource}{o^-}
% \newvariable{\OppSink}{i^-}
% 
% 
% \newvariable{\TheBundleMap}{f}
% \newvariable{\TheLocalTriv}{\phi}
% \newvariable{\TheCoordChange}{\phi}
% 
% \newvariable{\TheFibration}{\pi}
% \newvariable{\TheTotalSpace}{E}
% \newvariable{\TheBaseSpace}{X}
% \newvariable{\TheFibre}{F}
% \newvariable{\ThePartialLiftMap}{\bar{\TheMap}}
% \newvariable{\TheLiftMap}{\tilde{\TheMap}}
% 
% 
%   \newvariable{\TheCwComplex}{X}
%   \newvariable{\AltCwComplex}{Y}
%   \newvariable{\TheSubcomplex}{Y}
%   \newvariable{\TheSpanningTree}{\TheTree}
%   \newvariable{\AltSpanningTree}{\TheTree'}
%   \newvariable{\TheTreePoint}{t}
%   
%   \newcommand{\Map}{\pi}
%   \newcommand{\Total}{E}
%   \newcommand{\Base}{X}
%   \newcommand{\DerTotal}{\tilde{\Total}}
%   \newcommand{\DerBase}{\tilde{\Base}}
%   \newcommand{\DerMap}{\tilde{\Map}}
%   \newcommand{\Fibre}[1][]{F\IfEmptyThenElse{#1}{}{_{#1}}}
%   \newcommand{\TotalPoint}{\bullet_{\Total}}
%   \newcommand{\BasePoint}[1][\Base]{\bullet_{#1}}
%   \newvariable{\TheBasePoint}{P}
%   \newcommand{\TotalVertex}{\TotalCell_0}
%   \newcommand{\BaseVertex}{\BaseCell_0}
%   \newcommand{\TotalCell}{e}
%   \newcommand{\BaseCell}{x}
%   \newcommand{\face}{\leq}
%   \newcommand{\coface}{\geq}
%   \newcommand{\sface}{<}
%   \newcommand{\scoface}{>}
%   \newcommand{\MapLk}[2]{\Lk^{#1}\left(#2\right)}
%   \newcommand{\RelLk}[3]{\Lk^{#1}_{#3}\left(#2\right)}
  \newcommand{\Pair}[2]{(#1,#2)}
%   \newcommand{\NoParPair}[2]{#1,#2}
%   \newcommand{\CongClass}[1]{\left[#1\right]}
%   \newcommand{\EquiClass}[1]{\left[#1\right]}
%   \newcommand{\Top}[2]{\pi_{#1}#2}
%   \newcommand{\Eval}[2]{#1(#2)}
% 
%   \newcommand{\CovariantStar}[1]{{#1}_{*}}
%   \newcommand{\CovariantStarOf}[1]{\CovariantStar{#1}\OptIndexParentheses}
%   \newcommand{\ContravariantStar}[1]{#1^{*}}
%   \newcommand{\ContravariantStarOf}[1]{\ContravariantStar{#1}\OptIndexParentheses}
% 
%   \newcommand{\MInt}{\Int{\MOne}{\Zero}}
%   \newcommand{\BInt}{\Int{\MOne}{\One}}
%   \newcommand{\SimplexPoint}{x}
%   \newcommand{\Homotopy}{\Phi}
%   \newcommand{\Real}{t}
% 
%   \newcommand{\ColBase}{\Base'}
%   \newcommand{\ColTotal}{\Total'}
%   \newcommand{\IntermediateTotal}{\Total''}
%   \newcommand{\FreeBase}{x}
%   \newcommand{\FreeCoBase}{\tilde{\FreeBase}}
%   \newcommand{\FreeTotal}{e}
%   \newcommand{\FreeCoTotal}
% 
%   \newcommand{\RelLkVert}{V}
%  
% %  \newcommand{\gobbleone}[1]{}
% %  \newcommand{\SetOf}[2][\gobbleone]{\left\{#1 \mid #2\right\}}
% %  \newcommand{\Preim}[2]{#1^{-1}(#2)}
% %  \newcommand{\Union}[2][]{\bigcup_{#1}#2}
% %  \newcommand{\Intersection}[2][]{\bigcap_{#1}#2}
% %  \newcommand{\CardOf}[1]{\left|#1\right|}
%   \newcommand{\Restriction}[2]{#1\mid_{#2}}
%   \newcommand{\FinSequ}[3]{#1_{#2},\ldots,#1_{#3}}
% 
%   \newcommand{\TotalCoFace}{\bar{\TotalCell}}
%   \newcommand{\BaseCoFace}{\bar{\BaseCell}}
% 
% 
%   \newcommand{\Id}[1]{\mathrm{Id}_{#1}}
% 
%   \newcommand{\Ind}[2]{#1_{#2}}
%   \newcommand{\join}{*}
%   \newcommand{\boundary}[1]{\partial#1}
%
  \newvariable{\TheDim}{m}
%   \newcommand{\LowDim}{l}
%   \newcommand{\LOWdim}{k}
%   \newcommand{\HighDim}{n}
%   \newcommand{\TheSimplexDim}{k}
% 
%   \newcommand{\CovInd}{j}
%   \newcommand{\CovIndSet}{I}
%   \newcommand{\CovIndSubSet}{J}
% 
%   \newcommand{\TopInd}{n}
%   \newcommand{\TheInd}{i}
% 
% 
%   \newcommand{\FigOne}{%
%     \setlength{\unitlength}{3mm}
%     \begin{picture}(8,8)(0,0)
%       \path(0,6)(4,6)(8,8)(4,6)(8,4)
%       \put(4,2){\makebox[0pt][c]{$\downarrow$}}
%       \path(0,0)(8,0)
%     \end{picture}
%   }
% 
% 
%   \newcommand{\Set}{S}
%   \newvariable{\FreeGroup}{F}
%   \newvariable{\OutTor}{T}
%   \newcommand{\OutOf}{\Out\EvalAt}
%   \newvariable{\MapCl}{M}
  \newcommand{\GlOf}{\GL\OptIndexParentheses}
%   \newcommand{\SlOf}{\SL\OptIndexParentheses}
%   \newcommand{\PSlOf}{\PSL\OptIndexParentheses}
%   \newcommand{\SoOf}{\SO\EvalAt}
%   \newcommand{\AutOf}{\Aut\OptIndexParentheses}
%   \newcommand{\HomOf}{\Hom\OptIndexParentheses}
%   \newvariable{\TheSurface}{\Sigma}
%   \newvariable{\TheSurfaceUnivCover}{\UniversalCoverOf{\TheSurface}}
%   \newvariable{\TheSurfacePoint}{P}
%   \newvariable{\TheSurfaceBasePoint}{\underbar{\TheSurfacePoint}}
%   \newvariable{\TheSurfaceUnivCoverBasePoint}{\UniversalCoverOf{\TheSurfaceBasePoint}}
%   \newvariable{\AltSurfacePoint}{Q}
%   \newvariable{\AltSurfaceBasePoint}{\underbar{\AltSurfacePoint}}
%   \newvariable{\TheGenus}{g}
%   \newcommand{\SP}{\mathrm{Sp}}
%   \newcommand{\thegenus}{g}
%   \newcommand{\therank}{n}
%   \newcommand{\FTyp}[1]{F$_{#1}$}
%   \newcommand{\FPTyp}[1]{FP$_{#1}$}
% 
%   \newvariable{\TheGroup}{G}
%   \newvariable{\TheGroupModule}{M}
%   \newvariable{\AltGroup}{H}        
%   \newvariable{\TheGroupElement}{g}
%   \newvariable{\InvGroupElement}{\TheGroupElement^{-1}}
%   \newvariable{\AltGroupElement}{h}
%   \newvariable{\AltInvGroupElement}{\AltGroupElement^{-1}}
%   \newvariable{\TheSubgroupFamily}{\mathcal{H}}
%   \newvariable{\TheGroupElementVariable}{X}
% 
%   \newvariable{\TheReal}{t}
%   \newvariable{\AltReal}{s}
%   \newvariable{\LowReal}{r}
%   \newvariable{\HighReal}{s}
%         
%   \newvariable{\BCV}{\mathrm{BVC}}
% 
%   \newvariable{\TheNatural}{n}
%   \newvariable{\AltNatural}{m}
%   \newvariable{\LowNatural}{a}
%   \newvariable{\HighNatural}{b}
%       
% %
% 
% 
% 
% %  \newcommand{\Map}{\pi}
% %  \newcommand{\Total}{E}
% %  \newcommand{\Base}{X}
% %  \newcommand{\DerTotal}{\tilde{\Total}}
% %  \newcommand{\DerBase}{\tilde{\Base}}
% %  \newcommand{\DerMap}{\tilde{\Map}}
% %  \newcommand{\Fibre}[1][]{F\IfEmptyThenElse{#1}{}{_{#1}}}
% %  \newcommand{\TotalPoint}{\bullet_{\Total}}
% %  \newcommand{\BasePoint}{\bullet_{\Base}}
% %  \newcommand{\TotalVertex}{\TotalCell_0}
% %  \newcommand{\BaseVertex}{\BaseCell_0}
% %  \newcommand{\TotalCell}{e}
% %  \newcommand{\BaseCell}{x}
% %  \newcommand{\face}{\leq}
% %  \newcommand{\coface}{\geq}
% %  \newcommand{\sface}{<}
% %  \newcommand{\scoface}{>}
% %  \newcommand{\Link}{\mathrm{Lk}}
% %  \newcommand{\LinkOf}[2][]{\Link\IfEmptyThenElse{#1}{}{_{#1}}\left(#2\right)}
% %  \newcommand{\MapLk}[2]{\Link^{#1}\left(#2\right)}
% %  \newcommand{\RelLk}[3]{\Link^{#1}_{#3}\left(#2\right)}
% %  \newcommand{\Pair}[2]{(#1,#2)}
% %  \newcommand{\Top}[2]{\pi_{#1}#2}
% %  \newcommand{\Eval}[2]{#1(#2)}
% %
% %  \newcommand{\MInt}{\Int{\MOne}{\Zero}}
% %  \newcommand{\BInt}{\Int{\MOne}{\One}}
% %  \newcommand{\SimplexPoint}{x}
% %  \newcommand{\Homotopy}{\Phi}
% %  \newcommand{\Real}{t}
% %
% %  \newcommand{\ColBase}{\Base'}
% %  \newcommand{\ColTotal}{\Total'}
% %  \newcommand{\IntermediateTotal}{\Total''}
% %  \newcommand{\FreeBase}{x}
% %  \newcommand{\FreeCoBase}{\tilde{\FreeBase}}
% %  \newcommand{\FreeTotal}{e}
% %  \newcommand{\FreeCoTotal}
% %
% %  \newcommand{\RelLkVert}{V}
% % 
% %  \newcommand{\gobbleone}[1]{}
% %  \newcommand{\SetOf}[2][\gobbleone]{\left\{#1 \mid #2\right\}}
% %  \newcommand{\Preim}[2]{#1^{-1}(#2)}
% %  \newcommand{\Union}[2][]{\bigcup_{#1}#2}
% %  \newcommand{\Intersection}[2][]{\bigcap_{#1}#2}
% %  \newcommand{\CardOf}[1]{\left|#1\right|}
% %  \newcommand{\Restriction}[2]{#1\mid_{#2}}
% %  \newcommand{\FinSequ}[3]{#1_{#2},\ldots,#1_{#3}}
% %
% %  \newcommand{\TotalCoFace}{\bar{\TotalCell}}
% %  \newcommand{\BaseCoFace}{\bar{\BaseCell}}
% %
% %
% %  \newcommand{\Id}[1]{\mathrm{Id}_{#1}}
% %
% %  \newcommand{\Ind}[2]{#1_{#2}}
% %  \newcommand{\join}{*}
% %  \newcommand{\boundary}[1]{\partial#1}
% %
% %  \newcommand{\TheDim}{m}
% %  \newcommand{\LowDim}{l}
% %  \newcommand{\LOWdim}{k}
% %  \newcommand{\HighDim}{n}
% %
% %  \newcommand{\CovInd}{j}
% %  \newcommand{\CovIndSet}{I}
% %  \newcommand{\CovIndSubSet}{J}
% %
% %  \newcommand{\TopInd}{n}
% %  \newcommand{\TheInd}{i}
% %
% %
% %  \newcommand{\FigOne}{%
% %    \setlength{\unitlength}{3mm}
% %    \begin{picture}(8,8)(0,0)
% %      \path(0,6)(4,6)(8,8)(4,6)(8,4)
% %      \put(4,2){\makebox[0pt][c]{$\downarrow$}}
% %      \path(0,0)(8,0)
% %    \end{picture}
% %  }
% 
% 
% %
% % Bieri Strebel Theory
% %
% \newcommand{\BNSRsym}{\Sigma}
% \newcommand{\BNSR}[2][*]{{\BNSRsym}^{#1}\EvalAt{#2}}
% \newcommand{\BNSRcompl}[2][*]{{\BNSRsym}^{#1}\EvalAt{#2}^{\mathrm{c}}}
% \newcommand{\BS}[1]{\BNSRsym_{#1}\OptParentheses}
% \newcommand{\BScompl}[1]{\BNSRsym_{#1}^{\mathrm{c}}\OptParentheses}
% 
% 
% %
% % Linear Algebra
% %
% \newvariable{\TheVectorSpace}{V}
% \newvariable{\TheVectorSpaceSubset}{M}
% \newvariable{\TheBasisVector}{e}
% \newcommand{\ScalarProd}[3][]{\left\langle#2,#3\right\rangle_{#1}}
% % \newcommand{\ScalarProd}[2]{#1\cdot#2}
% \newcommand{\LinearSpan}[1]{\left\langle#1\right\rangle}
% \newvariable{\TheDualVectorSpace}{\DualOf{\TheVectorSpace}}
% 
% %
% % Groups
% %
% \newcommand{\SQ}{{SQ}}
\newvariable{\Houghton}{H}
% \newvariable{\TheHoughtonPermutation}{\pi}
% \newvariable{\FirstInt}{i}
% \newvariable{\SecondInt}{k}
% \newvariable{\Shift}{m}
\newvariable{\HoughtonBraid}{\Houghton^{\mathrm{br}}}
\newvariable{\SymmetricGroup}{\operatorname{Perm}}
% \newcommand{\OrientedEdgeToRel}{\mathrel{\rightarrow\!\!\!\!-}}
% \newcommand{\EdgeToRel}{\mathrel{-\!\!-}}
% \newvariable{\DihedralGroup}{D}
% \newvariable{\TheSymmetricGroup}{S}
% \newvariable{\TheAlternatingGroup}{A}
% 
% \newvariable{\TheX}{x}
% \newvariable{\InvX}{\bar{x}}
% \newvariable{\TheY}{y}
% \newvariable{\InvY}{\bar{y}}
% \newvariable{\TheFreeGroupElement}{w}
% 
% \newvariable{\TheKampenDiagram}{D}
% \newvariable{\AltKampenDiagram}{M}
% 
% \newcommand{\Commutator}[2]{\left[#1,#2\right]}
% \newcommand{\CommutatorSubgr}[1]{\Commutator{#1}{#1}}
% 
% \newvariable{\Vierergruppe}{\VVV}
% 
% \newcommand{\AbelianizationOf}[1]{#1^{\text{ab}}}
% 
% \newcommand{\StabilizerOf}{\operatorname{Stab}\OptIndexParentheses}
% 
% \newvariable{\TheType}{m}
% 
% \newcommand{\IA}{\operatorname{IA}\OptParentheses}
% 
% %
% % Calculus
% %
% \newvariable{\ThePosVector}{\mathbf{r}}
% \newvariable{\ThePlane}{P}
% \newvariable{\eee}{\mathrm{e}}
% 
% %
% % Braid groups and Configuration Spaces
% %
% \newvariable{\ThePositionSet}{T}
% \newvariable{\ThePositionSubset}{S}
% \newvariable{\AltPositionSubset}{\ThePositionSubset'}
% \newvariable{\ThePositionSubsetPoset}{\mathcal{S}}
% \newvariable{\TheConfigurationSpace}{C}
% \newvariable{\TheCoverConfigurationSpace}{\tilde{\TheConfigurationSpace}}
% \newvariable{\TheCenteredConfigurationSpace}{\TheCoverConfigurationSpace^{\Zero}}
\newvariable{\BraidGroup}{B}
% \newvariable{\PureBraidGroup}{P}
% \newvariable{\TheFixedPositionSubset}{\ThePositionSubset_{\Zero}}
% \newvariable{\ThePolygon}{P}
% \newvariable{\ThePosition}{\alpha}
% \newvariable{\AltPosition}{\beta}
% \newvariable{\ThirdPosition}{\gamma}
% \newvariable{\FourthPosition}{\delta}
% \newvariable{\BraidGroupFamily}{\mathcal{B}}
% \newvariable{\BraidGroupPresentation}{\mathcal{P}^B}
% \newvariable{\BraidGroupGenerator}{s}
% \newvariable{\TheSubsetPoset}{\Sigma}
% \newvariable{\TheSubsetPosetElement}{\sigma}
% \newvariable{\AltSubsetPosetElement}{\tau}
% \newvariable{\TheSubsetLattice}{\Sigma}
% \newvariable{\TheSubsetLatticeElement}{\sigma}
% \newvariable{\AltSubsetLatticeElement}{\tau}
\newvariable{\ThePosetElement}{\alpha}
\newvariable{\AltPosetElement}{\beta}
\newvariable{\ThirdPosetElement}{\xi}
% \newvariable{\TheEilenbergMaclaneSpace}{K}
% \newvariable{\TheEilenbergMaclaneCover}{\tilde{\TheEilenbergMaclaneSpace}}
% \iffalse
% \newvariable{}{}
% \newvariable{}{}
% \newvariable{}{}
% \newvariable{}{}
% \newvariable{}{}
% \newvariable{}{}
% \fi
% 
% 
% %
% % Complexes
% %
% \newvariable{\TheFlagComplex}{L}
% %\newvariable{\TheCoveringSpace}{X}
% %\newcommand{\CoveringSpaceOf}[1]{\tilde{#1}}
% \newcommand{\CAT}[1]{%
%   \ensuremath{\text{CAT}(#1)}%
% %  CAT(\ensuremath{#1})%
% }
% \newvariable{\TheCompactSubset}{C}
% \newvariable{\AltCompactSubset}{D}
% \newvariable{\TheCurvature}{\kappa}
% \newvariable{\TheTriangle}{\Delta}
% \newvariable{\TheComparisonTriangle}{\TheTriangle'}
% \newvariable{\NearestPointProjection}{\pi}
% \newvariable{\TheFlat}{F}
% 
% %
% % Combinatorial Morse Theory
% % 
% \newvariable{\ThePEComplex}{X}
% \newvariable{\TheCriticalValue}{c}
% \newcommand{\DescLinkOf}{\Lk^{\downarrow}\OptIndexParentheses}
% \newcommand{\AscLinkOf}{\Lk^{\uparrow}\OptIndexParentheses}
% \newcommand{\Height}{h}
% \newvariable{\TheCubeComplex}{X}
% \newvariable{\TheCube}{c}
\newvariable{\TheSimplex}{\sigma}
\newvariable{\AltSimplex}{\tau}
% \newvariable{\TheMorseFunction}{h}
% \newvariable{\AltMorseFunction}{f}
% \newvariable{\TheHeight}{s}
% \newvariable{\AltHeight}{t}
% \newvariable{\TheDescLinkUnion}{D}
% \newvariable{\TheDescConeUnion}{C}
% 
% \newvariable{\TheLivingSubcomplex}{L^{\star}}
% \newvariable{\TheDeadSubcomplex}{L^{\dagger}}
% 
% %
% % Combinatorics
% %
% \newindexedmap{\SizedPartitions}{P}
% 
% %
% % Algebra
% %
% \newvariable{\ThePolynomial}{P}
\newvariable{\TheField}{k}
% \newvariable{\TheBigField}{K}
% \newvariable{\TheRing}{R}
% \newvariable{\TheSuperField}{K}
% \newcommand{\PolynomialRing}[2][\TheIndeterminate]{%
%   #2\left[#1\right]
% }
% \newcommand{\Adjoint}[2]{\PolynomialRing[#2]{#1}}
% \newcommand{\IdealGenerated}[2][]{\left<#2\right>\IfEmptyThenElse{#1}{}{_{#1}}}
% \newvariable{\TheIndeterminate}{t}
% \newmap{\MetabelianGroupScheme}{M}
% \newvariable{\ThePrimeSet}{S}
% \newcommand{\OkaSet}{\Oka_{\ThePrimeSet}}
% \newmap{\BorelScheme}{B}
% \newvariable{\TheCharacter}{\chi}
% \newvariable{\AbelianGroup}{A}
% \newvariable{\adim}{i}
% \newvariable{\FiniteField}{\FFF}
% \newcommand{\AlgClosureOf}{\overline}
% \newvariable{\IndexSet}{I}
% 
% \newvariable{\TheIsomorphism}{\phi}
% 
% \newindexedmap{\MinimalPolynomial}{\mu}
% 
% \newcommand{\isomorphic}{\cong}
% 
% \newvariable{\KroneckerDelta}{\delta}
% 
% \newvariable{\relatesto}{\sim}
% 
% %
% % Linear Algebraic Groups
% %
% \newvariable{\TheLag}{G}
% \newvariable{\AltLag}{H}
% \newvariable{\TheLagElement}{g}
% \newvariable{\TheLagElementVar}{X}
% \newvariable{\TheMatrix}{M}
% \newvariable{\AltMatrix}{N}
% \newvariable{\TheBorelSubgroup}{B}
% \newvariable{\TheBorelSubgroupSet}{\mathcal{B}}
% \newcommand{\RadicalOf}{\operatorname{Rad}\EvalAt}
% \newcommand{\AnyThing}{\star}
% \newvariable{\TheLagMorphism}{\varphi}
% \newvariable{\TheChevalleyGroupScheme}{\mathcal{G}}
% \newvariable{\TheBorelSubgroupScheme}{\mathcal{B}}
% \newvariable{\TheGlobalFunctionField}{K}
% %
% % Lie Algebras
% %
% \newvariable{\TheLieAlgebra}{\mathfrak{G}}
% \newvariable{\AltLieAlgebra}{\mathfrak{H}}
% \newvariable{\TheLieElement}{\mathfrak{g}}
% \newvariable{\AltLieElement}{\mathfrak{h}}
% \newvariable{\TheCBHlaw}{\bullet}
% \newcommand{\LieBraket}[2]{\left[#1,#2\right]}
% %
% % Numbers
% %
\newvariable{\ThePrime}{p}
% \newvariable{\AltPrime}{q}
% \newvariable{\ThePrimePower}{q}
% 
% %
% % Homological Algebra
% %
% \newvariable{\TheProjectiveModule}{P}
% \newmap{\TheAugmentationMap}{\varepsilon}
% \newvariable{\TheTrivialAbelianGroup}{\Zero}
% \newcommand{\TheIntegers}{\ZZZ\OptExponent}
% \newcommand{\TheRationals}{\QQQ\OptExponent}
% \newvariable{\WholeNums}{\ZZZ}
% \newvariable{\TheModulus}{m}
% \newcommand{\CohomologicalDimensionOf}[1][]{\operatorname{cd}\IfEmptyThenElse{#1}{}{_{#1}}}
% \newcommand{\ChainComplex}[1][*]{
%   \operatorname{C}\IfEmptyThenElse{#1}{}{_{#1}}%
% \EvalAt}
% \newcommand{\KernelOf}{\ker\EvalAt}
% \newcommand{\ImageOf}{\im\EvalAt}
% %
% % Groups
% %
% \newcommand{\NormalClosureOf}[2][]{%
% %  \left\langle#2\right\rangle
%   \overline{#2}%
%   \IfEmptyThenElse{#1}{}{^{#1}}
% }
% \newvariable{\TheAmalgamFactor}{A}
% \newvariable{\AltAmalgamFactor}{B}
% \newvariable{\TheAmalgamSubgroup}{C}
% \newcommand{\TheTrivialGroup}{1}
% \newvariable{\TheTrivialElement}{1}
% \newvariable{\TheAbelianGroup}{Q}
% \newvariable{\TheNilpotentGroup}{N}
% \newvariable{\TheModule}{M}
% \newvariable{\TheTrivialModule}{\Zero}
% \newvariable{\TheInjection}{\iota}
\newvariable{\TheProjection}{\pi}
% \newvariable{\TheSection}{\sigma}
% \newvariable{\TheSeriesFactor}{M}
% %\newcommand{\GroupRing}[2][\ZZZ]{#1#2}
% %\newvariable{\TheGroupSubset}{B}
% %\newvariable{\AltGroupSubset}{B'}
% %\newmap{\TheGroupMeasure}{\mu}
% \newvariable{\CyclicGroup}{C}
% \newcommand{\TheInfCyclicGroup}{\CyclicGroup[\infty]}
% \newvariable{\TheFiniteGroup}{F}
% \newvariable{\TheFiniteGroupSubset}{K}
% \newvariable{\AltFiniteGroupSubset}{L}
% \newcommand{\subgroup}{\leq}
% \newcommand{\normalsubgroup}{\trianglelefteq}
% \newcommand{\strictnormalsubgroup}{\triangleleft}
% \newcommand{\freeprod}[1][]{*\IfEmptyThenElse{#1}{}{_{#1}}}
% \newvariable{\TheFactor}{F}
% \newvariable{\TheQuotient}{Q}
% \newvariable{\TheQuotientElement}{q}
% \newvariable{\TheGeneratingSet}{\Sigma}
% \newvariable{\TheGeneratingSetElement}{\sigma}
% \newvariable{\AltGeneratingSet}{\Xi}
% \newvariable{\TheGroupSubset}{S}
% \newvariable{\AltGroupSubset}{T}
% \newvariable{\TheSubgroup}{H}
% %\newvariable{\AltSubgroup}{\TheSubgroup'}
% \newvariable{\TheFirstSubgroup}{A}
% \newvariable{\TheFirstSubgroupElement}{a}
% \newvariable{\TheSecondSubgroup}{B}
% \newvariable{\TheSecondSubgroupElement}{b}
% \newvariable{\TheNormalSubgroup}{N}
% \newvariable{\TheNormalSubgroupElement}{n}
% \newvariable{\TheSubgroupIndex}{s}
% \newvariable{\TheSubgroupGenerator}{t}
% \newcommand{\TheGeneratedSubgroup}[1]{\left<#1\right>}
% \newvariable{\TheHomomorphism}{\varphi}
% \newcommand{\CosetOf}{\overline}
% 
% \newvariable{\TheIsoperimetricFunction}{\delta}
% 
% 
% \newvariable{\TheSolvabilityClass}{s}
% 
% \newindexedmap{\Conjugation}{\alpha}
% 
% \newcommand{\RightConjugate}{\ToThePower}
% \newcommand{\RightConjugateBy}[2][]{#2^{#1}}
% 
% \newvariable{\TheCayleyLoopLength}{l}
% 
% \newvariable{\TheKernel}{K}
% 
% \newvariable{\TheSubgroupElement}{h}
% \newcommand{\Inverse}[1]{#1^{-1}}
% \newcommand{\Omitted}[1]{\hat{#1}}
% 
% \newvariable{\TheCosetRepresentative}{r}
% \newvariable{\TheSubgroupComplementElement}{f}
% 
% \newcommand{\GeometricDimensionOf}{\operatorname{gd}}
% 
% %
% % Cayley graphs
% %
% 
% \newvariable{\CayleyGraph}{\Gamma}
% \newvariable{\TheGrowthFunction}{\beta}
% \newvariable{\AltGrowthFunction}{\TheGrowthFunction'}
% \newvariable{\TheGrowthRate}{\lambda}
% \newvariable{\AltGrowthRate}{\TheGrowthRate'}
% \newvariable{\TheStretchConst}{L}
% \newvariable{\TheShiftConst}{K}
% \newvariable{\TheConstant}{C}
% \newvariable{\AltConstant}{\TheConstant'}
% \newcommand{\weaklydominatedby}{\preceq}
% \newcommand{\weaklyequivalent}{\sim}
% \newvariable{\TheMaxLength}{l}
% \newmap{\CaleyLabel}{\TheGeneratingSetElement}
% \newcommand{\CayleyLabelOf}[1]{\TheGeneratingSetElement[#1]}
% 
% \newvariable{\TheRightQuotientSpace}{X}
% \newvariable{\TheRightQuotientVertex}{x}
% 
% \newvariable{\ThePathSet}{\mathcal{P}}
\newvariable{\ThePath}{p}
% \newvariable{\PathSpace}{\mathcal{P}}
% \newvariable{\ThePathLift}{\tilde{\ThePath}}
% \newvariable{\AltPath}{q}
% \newvariable{\TheSpecialPath}{\gamma}
% \newvariable{\AltSpecialPath}{\delta}
% \newcommand{\EndPointOf}[1]{\overline{#1}}
% \newvariable{\ThePathPairSet}{\Pi}
% \newcommand{\pathconcat}{\mathbin{\rightarrow\!\!\!\!-}}
% \newvariable{\ThirdPath}{r}
% \newcommand{\ReversalOf}[1]{#1^{\mathrm{rev}}}
% 
% \newcommand{\NEndsOf}{\operatorname{e}\EvalAt}
% \newvariable{\TheRelation}{r}
% \newvariable{\TheRelator}{R}
% \newvariable{\TheRelationSet}{R}
% \newvariable{\AltRelationSet}{R'}
% \newvariable{\TheTwoCellFamily}{\mathcal{D}}
% \newindexedmap{\CayleyComplex}{\CayleyGraph}
% \newvariable{\ThePresentationComplex}{K}
% 
% \newvariable{\TheConvexity}{c}
% 
% %
% % Trees
% %
% \newvariable{\TheTree}{T}
% \newvariable{\TheTreeAutomorphism}{\varphi}
% \newvariable{\AltTreeAutomorphism}{\psi}
% \newvariable{\TheAxis}{C}
% \newvariable{\ForwardEnds}{\boundary_\infty^+}
% \newvariable{\BackwardEnds}{\boundary_\infty^-}
% 
% %
% % Words
% %
% \newvariable{\TheAlphabet}{\mathcal{A}}
% \newvariable{\AltAlphabet}{\mathcal{B}}
% \newcommand{\LanguageOver}[1]{#1^{*}}
% \newvariable{\TheSign}{\varepsilon}
% \newvariable{\TheWord}{w}
% \newvariable{\ThePiece}{b}
% \newvariable{\AltWord}{u}
% \newvariable{\ThirdWord}{v}
% \newvariable{\TheLetter}{a}
% \newvariable{\AltLetter}{b}
% \newvariable{\ThirdLetter}{c}
% \newvariable{\ForthLetter}{d}
% \newvariable{\TheSpecialLetter}{s}
% \newvariable{\AltSpecialLetter}{t}
% \newvariable{\TheWordLength}{r}
% \newvariable{\AltWordLength}{s}
% \newcommand{\WordLengthOf}[2][]{%
%   \IfEmptyThenElse{#1}{%
%     \AbsValue{#2}
%   }{
%     \AbsValue{#2}_{#1}
%   }
% }
% 
% 
% \newcommand{\ReducedWordOf}{\overline}
% \newcommand{\RepresentativeOf}{\overline}
% \newvariable{\TheTransversal}{T}
% 
% \newcommand{\LengthOf}{\WordLengthOf}
% 
% %
% % topological Groups
% %
% \newvariable{\TheTopologicalGroup}{G}
% \newvariable{\TheTopologicalGroupQuotient}{Q}
% \newvariable{\TheCompactGroupSubset}{K}
% \newvariable{\TheUnitaryRepresentation}{\rho}
% 
% %
% % G-Sets
% % 
% \newvariable{\TheGSet}{X}
% \newvariable{\TheGSetElement}{x}
% \newvariable{\TheGSubset}{Y}
% \newvariable{\AltGSubset}{Z}
% \newmap{\TheGSetMeasure}{\mu}
% \newvariable{\TheFolnerSubset}{F}
% 
% 
% %
% % Measure Theory
% %
% \newvariable{\TheMeasure}{\mu}
% \newvariable{\TheSubsetFamily}{\mathcal{M}}
% 
% %
% % Pinched Braids
% %
% \newvariable{\ThePBraid}{\alpha}
% \newvariable{\AltPBraid}{\beta}
% \newcommand{\PIndOf}[1]{\ind\EvalAt{#1}}
% \newvariable{\HBMonoid}{M^{\mathrm{br}}}
% \newvariable{\HBSubMonoid}{T}
% \newvariable{\BasePBraid}{t}
% \newvariable{\PBraidSpace}{X}
% \newcommand{\PBraidSublevel}[2][]{\PBraidSpace\IfNonEmpty{#1}{_{#1}}\EvalAt{#2}}
% \newvariable{\BasePBraidProd}{\mathbf{t}}
% \newvariable{\ThePBraidShift}{\rho}
% \newvariable{\TheBraidIndex}{m}
% \newcommand{\TheBraidLink}[2][]{L\IfNonEmpty{#1}{_{#1}}^{#2}}
% \newcommand{\OneBar}{\bar{\One}}
% \newcommand{\TwoBar}{\bar{\Two}}
% \newvariable{\TheIndexBar}{\bar{\TheIndex}}
% \newcommand{\TheBraidIndexBar}{\bar{\TheBraidIndex}}
% \newvariable{\TheBraidLinkBase}{L'}
% \newvariable{\TheBraidLinkBaseDef}{L^{*}}
% \newvariable{\TheBraidLinkExtension}{L''}
% \newvariable{\TheBraidVertex}{\ThePBraid}
% \newvariable{\AltBraidVertex}{\AltPBraid}
% \newcommand{\RunsOf}{R\EvalAt}
% \newvariable{\ThePLinkVertex}{v}
% 
% %
% %
% %
% \newcommand{\InfinitesimalElementOf}[1]{\diff#1}
% \newvariable{\TheFirstCoordinate}{x}
% \newcommand{\TheFirstInfElement}{\InfinitesimalElementOf{\TheFirstCoordinate}}
% \newvariable{\TheSecondCoordinate}{y}
% \newcommand{\TheSecondInfElement}{\InfinitesimalElementOf{\TheSecondCoordinate}}
% \newvariable{\TheThirdCoordinate}{z}
% \newcommand{\TheThirdInfElement}{\InfinitesimalElementOf{\TheThirdCoordinate}}
% \newvariable{\TheArcLength}{s}
% \newcommand{\TheArcLengthInfElement}{\InfinitesimalElementOf{\TheArcLength}}
% \newvariable{\TheArea}{A}
% \newcommand{\TheAreaInfElement}{\diff\TheArea}
% %
% % Set Theory
% %
% \newvariable{\TheSet}{M}
% \newvariable{\TheSetElement}{m}
% \newvariable{\AltSet}{N}
% \newvariable{\AltSetElement}{n}
% \newvariable{\TheSubset}{S}
% \newvariable{\TheSubsetElement}{s}
% \newvariable{\AltSubset}{T}
% \newvariable{\TheFilterElement}{F}
% \newvariable{\AltFilterElement}{H}
% \newvariable{\TheFilter}{\mathcal{F}}
% \newvariable{\AltFilter}{\mathcal{H}}
% \newvariable{\TheUltrafilter}{\mathcal{U}}
% \newvariable{\TheCofiniteFilter}{\mathcal{CF}}
% \newvariable{\TheCoinitialFilter}{\mathcal{CI}}
% \newcommand{\UltraLimit}[1][]{#1\text{-}\Limit}
% \newcommand{\FilterLimit}{\UltraLimit}
% \newvariable{\TheUltraLimit}{\TheSequenceTerm}
% \newvariable{\TheFilterLimit}{\TheSequenceTerm}
% \newcommand{\PowerSetOf}{\mathcal{P}\EvalAt}
% \newvariable{\TheIdentity}{\mathrm{id}}
% 
% %
% % Ordered Sets
% %
\newcommand{\FiberSymbol}{\mathfrak{F}}
\newcommand{\FiberOver}[2][]{%
  \IfEmptyThenElse{#1}{
    \mathop{\FiberSymbol}\left(#2\right)
  }{
    \mathop{\FiberSymbol}\nolimits_{#1}\left(#2\right)
  }
}
\newvariable{\ThePoset}{P}
\newvariable{\AltPoset}{Q}
% \newvariable{\TheToset}{T}
% \newvariable{\ThePoChain}{C}
% \newvariable{\AltPoChain}{D}
% \newvariable{\TheToChain}{C}
% \newvariable{\AltToChain}{D}
% \newvariable{\TheAntiChain}{A}
% %\newvariable{\TheSegment}{I}
% \newvariable{\TheCosegment}{F}
% %\newvariable{\TheToElement}{t}
% %\newvariable{\AltToElement}{s}
% \newvariable{\TheDirectedSet}{D}
% \newvariable{\TheDirectedSetElement}{\alpha}
% \newvariable{\AltDirectedSetElement}{\beta}
% \newvariable{\HighDirectedSetElement}{\beta}
% \newvariable{\LowDirectedSetElement}{\alpha}
% 
\newvariable{\ThePosetMap}{f}
% \newcommand{\PosetFibreOfAt}[2]{#1\rmod#2}
% \newcommand{\PosetCofibreOfAt}[2]{#2\lmod#1}
% \newvariable{\TheCell}{p}
% \newvariable{\AltCell}{q}
\newvariable{\isfaceof}{\preceq}
\newvariable{\isstrictfaceof}{\prec}
% \newcommand{\OppPosetOf}[1]{#1^{\mathrm{op}}}
% \newvariable{\TheClosedSubposet}{U}
% \newcommand{\weakorder}{\preceq}
% 
% %
% % Analysis
% %
% \newvariable{\TheForm}{\omega}
% \newvariable{\Gradient}{\nabla}
% \newvariable{\TheCurve}{\vec{c}}
% \newvariable{\TheParametrization}{\Phi}
% \newvariable{\TheDomain}{D}
% \newvariable{\TheRange}{R}
% \newvariable{\TheEpsilon}{\varepsilon}
% \newvariable{\TheDelta}{\delta}
% \newvariable{\TheSequenceTerm}{a}
% \newvariable{\TheSequence}{\FamOf{\TheSequenceTerm[\TheIndex]}}
% \newvariable{\TheInterval}{I}
% \newvariable{\AltInterval}{J}
% \newvariable{\TheHilbertSpace}{\mathcal{H}}
% \newcommand{\LSpaceOf}[2][]{L^{#1}\left(#2\right)}
% \newcommand{\LTwoOf}[1]{\LSpaceOf[\Two]{#1}}
% \newvariable{\TheUnitVector}{\mathbf{u}}
% \newcommand{\UnitaryGroup}[1][]{%
%   \operatorname{U}%
%   \IfEmptyThenElse{#1}{}{_{#1}}
% }
% \newindexedmap{\SpecialOrthogonalGroup}{\operatorname{SO}}
% \newvariable{\TheVectorField}{\vec{V}}
% 
% 
% \newmap{\TheLeftProbabilityMeasure}{\mu}
% \newmap{\TheRightProbabilityMeasure}{\TheLeftProbabilityMeasure^{-}}
% \newmap{\TheBiProbabilityMeasure}{\tilde{\TheLeftProbabilityMeasure}}
% \newcommand{\MeasureElement}[2][]{\IfEmptyThenElse{#1}{\diff#2}{\diff_{#1}#2}}
% 
% \newcommand{\vol}{\operatorname{vol}}
% \newcommand{\Vol}{\vol\EvalAt}
% \newvariable{\Ball}{\BBB}
% 
% \newcommand{\BoundedFunctionsOn}{\operatorname{L}\EvalAt}
% \newindexedmap{\CharacteristicFunction}{\chi}
% \newindexedmap{\TheBoundedFunction}{f}
% \newvariable{\TheArgument}{x}
% 
% \newcommand{\BigOOf}{O\EvalAt}
% 
% \newvariable{\TheCoefficient}{a}
% \newvariable{\AltCoefficient}{b}
% 
% \newvariable{\TheComplexNum}{z}
% \newcommand{\RealOf}{\Re\EvalAt}
% \newcommand{\ImOf}{\Im\EvalAt}
% \newcommand{\ConjugateOf}{\overline}
% 
% \newvariable{\TheComplex}{z}
% \newvariable{\AltComplex}{z'}
% %
% % Topology
% %
\newvariable{\TheNumberOfComponents}{k}
% \newcommand{\MappingConeOf}{%
%   \mathrm{MC}\EvalAt
% }
% \newcommand{\CoverOf}[1]{\tilde{#1}}
% \newvariable{\TheCover}{\mathcal{A}}
% \newvariable{\TopSpacesCategory}{\mathbf{Top}}
% \newvariable{\SetsCategory}{\mathbf{Set}}
\newvariable{\TheSpace}{X}
% \newvariable{\TheCellComplex}{X}
% \newvariable{\AltCellComplex}{Y}
% \newcommand{\SkeletonOf}[2][]{#2^{(#1)}}
% \newvariable{\TheSpacePoint}{x}
% \newvariable{\TheSpaceBasePoint}{\underbar{\TheSpacePoint}}
% \newvariable{\TheCoveringSpace}{\bar{\TheSpace}}
% \newvariable{\TheCoveringSpacePoint}{\bar{\TheSpacePoint}}
% \newvariable{\TheCoveringSpaceBasePoint}{\bar{\TheSpaceBasePoint}}
% \newvariable{\TheCoveringProjection}{\pi}
% \newvariable{\ThePathCover}{\bar{\ThePath}}
% \newvariable{\AltPathCover}{\bar{\AltPath}}
% \newcommand{\UniversalCoverOf}[1]{\tilde{#1}}
% \newvariable{\TheUniversalCover}{\UniversalCoverOf{\TheSpace}}
% \newvariable{\TheUniversalCoverProjection}{\UniversalCoverOf{\TheCoveringProjection}}
% \newvariable{\TheUniversalCoverBasePoint}{\UniversalCoverOf{\TheSpaceBasePoint}}
% \newcommand{\DeckTransformations}{\mathrm{Cov}}
% \newcommand{\DeckTransformationsOf}[2][]{\DeckTransformations\Parentheses{#2\IfEmptyThenElse{#1}{}{\rmod#1}}}
% \newvariable{\AltSpace}{Y}
% \newvariable{\AltSpacePoint}{y}
% \newvariable{\AltSpaceBasePoint}{\underbar{\AltSpacePoint}}
% \newvariable{\AltSpaceComponent}{\AltSpace^{\Zero}}
\newvariable{\ThePoint}{x}
% \newvariable{\AltPoint}{y}
% \newvariable{\ThirdPoint}{z}
% \newvariable{\ThirdSpace}{Z}
% \newvariable{\ThirdSpacePoint}{z}
% \newvariable{\ThirdSpaceBasePoint}{\underbar{\ThirdSpacePoint}}
% \newvariable{\ThePlanePoint}{P}
% \newvariable{\AltPlanePoint}{Q}
% \newvariable{\ThePointFamilyTerm}{\ThePoint}
% \newvariable{\ThePointFamily}{\FamOf[\TheSetElement\in\TheSet]{\ThePointFamilyTerm[\TheSetElement]}}
% \newvariable{\TheCompactSpace}{C}
% \newvariable{\AltCompactSpace}{D}
% \newvariable{\TheCompactPoint}{x}
% \newvariable{\AltCompactPoint}{y}
% \newvariable{\TheCompactPointFamilyTerm}{\TheCompactPoint}
% \newvariable{\TheCompactPointFamily}{\FamOf[\TheSetElement\in\TheSet]{\TheCompactPointFamilyTerm[\TheSetElement]}}
% \newvariable{\TheOpenSet}{U}
% \newvariable{\TheCoveringOpenSet}{\TheOpenSet'}
% \newvariable{\TheOpenComponent}{\TheOpenSet^{\Zero}}
% \newvariable{\TheOpenSetElement}{u}
% \newvariable{\AltOpenSetElement}{v}
% \newvariable{\AltOpenSet}{V}
% \newvariable{\TheOpenNeighbourhood}{\TheOpenSet}
% \newvariable{\AltOpenNeighbourhood}{\AltOpenSet}
\newvariable{\TheFunction}{f}
% \newvariable{\AltFunction}{h}
% \newvariable{\TheHomotopy}{\Phi}
% \newvariable{\AltHomotopy}{\Psi}
% \newvariable{\TheHomeomorphism}{\zeta}
% \newvariable{\AltHomeomorphism}{\xi}
% \newcommand{\Sphere}{\mathbb{S}\OptExponent}
% \newvariable{\Circle}{\mathbb{S}^{\One}}
\newvariable{\TheSphere}{S}
% \newvariable{\AltSphere}{\TheSphere'}
% \newvariable{\TheCircle}{C}
% \newcommand{\SphericalizationOf}{\TheSphere\OptIndexParentheses}
% \newcommand{\Disc}{\mathbb{D}\OptExponent}
% \newvariable{\TheDisc}{D}
% \newvariable{\NorthMap}{\nu}
% \newvariable{\SouthMap}{\sigma}
% \newvariable{\TheNet}{n}
\newcommand{\ClosureOf}{\overline}
% \newvariable{\TheOpenCover}{\mathcal{U}}
% \newvariable{\TheNerve}{N}
% \newcommand{\NerveOf}[1]{\mathcal{N}\EvalAt{#1}}
% \newmap{\EndsOf}{\boundary_\infty}
% \newvariable{\TheSetOfEnds}{\mathcal{E}}
% \newcommand{\HomotopyClasses}[2]{\left[#1;#2\right]}
% \newcommand{\ConeOf}{\operatorname{Cone}\EvalAt}
% \newvariable{\homotopyequiv}{\backsimeq}
% 
\newcommand{\RealizationOf}[1]{\left|#1\right|}
\newvariable{\TheSimplicialComplex}{K}
% \newvariable{\AltSimplicialComplex}{L}
% 
% \newvariable{\TheComponent}{W}
% \newcommand{\ConnectedComponentOf}[1]{{#1}^{\Zero}}
% 
% \newcommand{\MappingClassesOf}{\mathcal{M}\EvalAt}
% \newvariable{\TheTorus}{T}
% \newvariable{\TheTorusBasePoint}{\underbar{t}}
% 
% \newvariable{\TheRepresentativeSet}{R}
% \newvariable{\TheCycle}{c}
% \newvariable{\AltCycle}{c'}
% \newvariable{\TheBoundedRegion}{B}
% 
% \newcommand{\ContFromTo}[2]{\mathrm{C}\left(#1,#2\right)}
% 
% %
% % Geodesic Homology
% %
% \newindexedmap{\TheGeodesicCycle}{\zeta}
% \newindexedmap{\TheZeroCycle}{\zeta^{\Zero}}
% \newcommand{\TheZeroCycleOf}{\TheZeroCycle\EvalAt}
% \newindexedmap{\TheOneCycle}{\zeta^{\One}}
% \newindexedmap{\AltOneCycle}{\xi^{\One}}
% \newcommand{\TheOneCycleOf}{\TheOneCycle\EvalAt}
% \newvariable{\TheTwoChain}{\zeta^{\Two}}
% \newvariable{\TheCarrier}{C}
% \newvariable{\RotationAround}{\mathrm{rot}}
% \newvariable{\TheTriangulation}{\mathcal{T}}
% \newvariable{\AltTriangulation}{\mathcal{T}'}
% \newvariable{\TheArc}{A}
% \newvariable{\AltArc}{\TheArc'}
% \newvariable{\TheInterior}{I}
% \newvariable{\TheStereographicEmbedding}{\iota}
% \newvariable{\TheBrokenLine}{\beta}
% \newvariable{\AltBrokenLine}{\pi}
% \newvariable{\TheBrokenGeodesic}{\gamma}
% \newvariable{\TheSquareCover}{Q}
% \newvariable{\TheBoundaryPartition}{\mathcal{P}}
% \newvariable{\TheDrivewaySet}{\mathcal{D}}
% 
% %
% % Metric Spaces
% %
% \newvariable{\TheNormManifold}{M}
% \newvariable{\TheMetricSpace}{X}
% \newvariable{\AltMetricSpace}{Y}
% \newvariable{\TheMetricSubspace}{X'}
% \newvariable{\TheMetricSpacePoint}{x}
% \newvariable{\AltMetricSpacePoint}{y}
% \newvariable{\TheMetric}{d}
% \renewcommand{\TheMetricOf}{\TheMetric\OptIndexDoubleArg}
% \newvariable{\TheBDMap}{\varphi}
% \newvariable{\TheRadius}{r}
% \newvariable{\TheRadiusConst}{R}
% \newvariable{\TheBigRadius}{R}
% \newvariable{\TheSmallRadius}{r}
\newvariable{\TheBall}{B}
% \newvariable{\TheClosedBall}{\bar{\TheBall}}
% \newcommand{\TheClosedBallAround}{\TheClosedBall\OptIndexParentheses}
% \newvariable{\TheOpenBall}{\TheBall}
% \newcommand{\TheOpenBallAround}{\TheOpenBall\OptIndexParentheses}
% \newcommand{\DistanceOf}[3][]{%
%   \TheMetric
%   \IfEmptyThenElse{#1}{}{_{#1}}%
%   \EvalAt{#2,#3}
% }
% 
% \newvariable{\TheMetricSpaceSubset}{Y}
% 
% \newvariable{\TheSimilarity}{\sigma}
% \newvariable{\TheIsometry}{\lambda}
% 
% \newvariable{\TheUnivCoverIsometry}{\CoverOf{\TheIsometry}}
% \newvariable{\DisplacementMap}{D}
% \newvariable{\Displacement}{D}
% \newvariable{\TheTranslation}{\tau}
% \newvariable{\TranslationDistance}{\tau}
% \newvariable{\TranslationLength}{\underline{\tau}}
% \newvariable{\TheDiameter}{D}
% \newcommand{\DiameterOf}[1][]{\operatorname{diam}\IfEmptyThenElse{#1}{}{_{#1}}\EvalAt}
% 
% \newcommand{\MinSetOf}[1]{\operatorname{Min}\EvalAt{#1}}
% 
% 
% \newvariable{\TheTime}{t}
% 
% \newvariable{\TheGeodesic}{\gamma}
% \newvariable{\AltGeodesic}{\gamma'}
% \newcommand{\pathto}{\longrightarrow}
% 
% \newcommand{\GeodesicSegment}[3][]{%
%   \ClosedInterval{#2}{#3}%
%   \IfEmptyThenElse{#1}{}{_{#1}}
% }
% 
% \newvariable{\TheGeodesicSet}{l}
% 
% \newvariable{\TheLength}{\ell}
% 
% \newvariable{\TheAngle}{\alpha}
% \newvariable{\AltAngle}{\beta}
% \newvariable{\ThirdAngle}{\gamma}
% \newvariable{\TheSideLength}{a}
% \newvariable{\AltSideLength}{b}
% \newvariable{\ThirdSideLength}{c}
% 
% \newvariable{\TheQuasiIsometry}{\varphi}
% 
% \newcommand{\TheBigStabilizerOf}[2][]{%
%   \IfEmptyThenElse{#1}{%
%     \overline{\mathrm{Stab}}\EvalAt{#2}
%   }{%
%     \overline{\mathrm{Stab}}_{#1}\EvalAt{#2}
%   }
% }
% 
% %
% % Misc
% %
% \newvariable{\TheCenter}{c}
% \newcommand{\TheUnitInterval}{\III\OptExponent}
% \newcommand{\TheUnitBall}{\BBB\OptExponent}
% \newcommand{\TheUnitSphere}{\SSS\OptExponent}
% \newcommand{\EuclideanSpace}{\EEE\OptExponent}
% \newcommand{\TheUnitTorus}{\TTT\OptExponent}
% \newvariable{\TheOpenPositiveReals}{\RRR_{\geq\Zero}^{\infty}}
% \newvariable{\TheIndexSet}{I}
% \newvariable{\AltIndexSet}{J}
% \newcommand{\DummyArg}{-}
% \newcommand{\DummyEntry}{\star}
% \newvariable{\TheIndexSubset}{K}
% \newvariable{\AltIndexSubset}{L}
% 
% \newvariable{\TheMiddleDisc}{C_{\Zero}}
% \newvariable{\TheAnnulus}{R}
% \newparexpvariable{\TheAnnulusDisc}{C}
% \newvariable{\AltMiddleDisc}{\tilde{C}_{\Zero}}
% \newvariable{\AltAnnulus}{\tilde{R}}
% \newparexpvariable{\AltAnnulusDisc}{\tilde{C}}
% 
% \newvariable{\TheLimit}{L}
% \newvariable{\AltLimit}{a}
% 
% %
% % Thompsons groups
% %
% \newvariable{\TheTopTree}{T^{\LabelTop}}
% \newvariable{\TheBotTree}{T^{\LabelBot}}
% \newvariable{\TheCantorSet}{\mathcal{C}}
% \newvariable{\TheCantorHomeo}{f}
% \newvariable{\TheLeftEnd}{0}
% \newvariable{\TheRightEnd}{1}
% \newvariable{\TheExpression}{A}
% \newvariable{\AltExpression}{B}
% \newvariable{\ThirdExpression}{C}
% \newvariable{\ForthExpression}{D}
% \newvariable{\ThTee}{T}
% \newcommand{\ThPlOf}[1]{%
%   F(\OneHalf,#1)
% %\PlOf[\Adjoint{\TheIntegers}{\OneHalf},\ToThePower{\Two}{\TheIntegers}]{\TheOpenPositiveReals}
% }
% \newvariable{\ThEff}{F}
% \newvariable{\ThPresentation}{\tilde{\ThEff}}
% \newcommand{\ThompsonsGroup}[1]{#1}
% \newexpvar{\EffGenerator}{x}
% \newexpvar{\EffCantorHomeo}{\xi}
% \newexpvar{\ThEffElement}{f}
% \newexpvar{\AltEffElement}{g}
% \newexpvar{\ThirdEffElement}{h}
% \newcommand{\ThPlLine}{\ThPlOf{\TheOpenPositiveReals}}
% \newvariable{\ThPlLineElement}{\varphi}
% \newvariable{\AltPlLineElement}{\psi}
% \newcommand{\ThPlInt}{\ThPlOf{\TheUnitInterval}}
% \newvariable{\ThPlIntElement}{\varphi}
% \newexpvar{\ThPlLineGenerator}{\xi}
% \newvariable{\ThPlAltInt}{\ThPlOf{\AltInterval}}
% \newvariable{\ThePositiveCone}{P}
% \newvariable{\TheThLabel}{q}
% \newvariable{\ThEffPositiveMonoid}{P}
% \newvariable{\ThEffCover}{Y}
% \newvariable{\ThEffPositiveCover}{\ThEffCover[+]}
% \newexpvar{\ThEffComplex}{X}
% \newexpvar{\ThEffPosComplex}{{\ThEffComplex_+}}
% \newexpvar{\ThEffNegComplex}{{\ThEffComplex_-}}
% \newvariable{\ThPosBoundaryOf}{\partial^+}
% \newvariable{\ThNegBoundaryOf}{\partial^-}
% \newvariable{\ThPMBoundaryOf}{\partial^-}
% \newvariable{\ThEffCube}{\mathbf{\TheThLabel}}
% \newvariable{\ThEffEdge}{\TheThLabel}
% \newvariable{\ThEffFace}{\mathbf{p}}
% \newvariable{\ThFaceEdge}{p}
% \newvariable{\ThEffModel}{Z}
% \newvariable{\ThHomotopyEquiv}{\pi}
% \newvariable{\ThEffBit}{\TheEpsilon}
% 
% \newvariable{\OurKFOne}{Y}
% \newvariable{\ThePointSet}{S}
% 
% \newvariable{\TheOnePositiveCount}{c_{\One}^{+}}
% \newvariable{\TheOneNegativeCount}{c_{\One}^{-}}
% \newvariable{\TheZeroCount}{c_{\Zero}}
% 
% \newcommand{\TI}{\textbf{I}}
% \newcommand{\TR}{\textbf{R}}
% \newcommand{\TN}{\textbf{N}}
% \newcommand{\TL}{\textbf{L}}
% \newvariable{\TheWidth}{w}
% \newvariable{\ThEffLength}{\ell}
% \newvariable{\PathLength}{L}
% 
% \newvariable{\TheTreeDiagram}{\mathfrak{t}}
% 
% \newcommand{\OurLeftVertex}[1][]{l}
% \newcommand{\OurCenterVertex}[1][]{c}
% \newcommand{\OurRightVertex}[1][]{r}
% \newcommand{\AltLeftVertex}[1][]{l'}
% \newcommand{\AltRightVertex}[1][]{r'}
% %\newvariable{\TheLeft}{L}
% %\newvariable{\TheRight}{R}
% %\newvariable{\TheCenter}{C}
% \newvariable{\CutLeftVertex}{h_l}
% \newvariable{\CutRightVertex}{h_r}
% \newvariable{\OurCutVertex}{g}
% \newvariable{\LeftSidedVertex}{\CutLeftVertex'}
% 
% \newcommand{\OurCriticalThEffElement}[1][]{g_{(#1)}}
% \newvariable{\TheFirst}{F}
% \newvariable{\TheLast}{L}
% 
% \newvariable{\SimpleEffElement}{h}
% 
% \newcommand{\LeftHalfOf}{L\OptIndexParentheses}
% \newcommand{\RightHalfOf}{R\OptIndexParentheses}
% 
% \newcommand{\TopForestOf}{\mathcal{T}\OptIndexParentheses}
% \newcommand{\BotForestOf}{\mathcal{B}\OptIndexParentheses}
% \newvariable{\TheForestDiagram}{\mathfrak{f}}
% \newvariable{\AltForestDiagram}{\mathfrak{g}}
% \newvariable{\TheTopForest}{T}
% \newvariable{\TheBotForest}{B}
% 
% \newvariable{\TheConvexityBound}{C}
% 
% 
% %
% % PL-Homeomorphism Groups
% %
% \newcommand{\PlOf}[1][]{
%   \operatorname{PL}\IfEmptyThenElse{#1}{}{_{#1}}\EvalAt
% }
% 
% \newvariable{\TheDecomposition}{\mathcal{I}}
% \newvariable{\AltDecomposition}{\mathcal{J}}
% \newvariable{\TheSDI}{I}
% \newvariable{\AltSDI}{J}
% \newvariable{\TheStandardDyadicForest}{\mathcal{F}^{(\Two)}}
% \newvariable{\TheDyadicForest}{\mathcal{F}^{(\Two)}}
% %
% % Tree Sets
% %
% \newvariable{\TheTreeSet}{T}
% \newcommand{\TheTreeSetInv}[1][]{%
%   \IfEmptyThenElse{#1}{%
%     (-)
%   }{%
%     \overline{#1}
%   }
% }
% \newcommand{\TheTreeSetRel}{\mathrel{\rightarrow\!\!\!\!-}}
% \newvariable{\TheTreeSetElement}{t}
% \newvariable{\AltTreeSetElement}{t'}
% \newcommand{\TheTreeSetInt}[2]{\left[#1,#2\right]}
% \newcommand{\TheTreeSetEquiv}{\sim}
% \newvariable{\TheTreeUpperHalf}{\TheTreeSet}
% 
% %
% % Dicks and Dunwoody Theory
% %
% \newvariable{\TheGroupHalfSet}{\mathcal{H}}
% \newcommand{\HalfComplementOf}[1]{\overline{#1}}
% \newvariable{\TheGroupHalf}{U}
% \newvariable{\AltGroupHalf}{V}
% \newvariable{\TheMin}{m}
% \newvariable{\TheHalfEquiv}{\cong}
% \newvariable{\TheSpecialHalf}{\TheGroupHalf[\Zero]}
% 
% %
% % Stallings Folds
% %
% \newvariable{\TheGLabeling}{\phi}
% \newvariable{\TheGLabelHom}{\phi}
% \newvariable{\TheCoreGraphCategory}{\mathbf{Graphs}}
% \newvariable{\TheSmallGraphCategory}{\TheCoreGraphCategory^*}
% \newvariable{\TheHomotopyGraphCategory}{\mathbf{M-Graphs}}
% \newvariable{\TheSmallHomotopyGraphCategory}{\TheHomotopyGraphCategory^*}
% \newcommand{\CoreOf}[1]{\mathrm{core}\EvalAt{#1}}
% \newvariable{\TheRose}{R}
% \newvariable{\ThePedal}{l}
% \newvariable{\TheSubdivRose}{\overline{\TheRose}}
% \newvariable{\TheHomotopyLabelling}{\vartheta}
% \newvariable{\AltHomotopyLabelling}{\tau}
% \newvariable{\TheGraphHomeomorphism}{\rho}
% \newvariable{\TheMetrics}{\mathbf{\Sigma}}
% \newvariable{\TheNDMetrics}{\topcirc{\mathbf{\Sigma}}}
% \newvariable{\TheBordifiedMetrics}{\hat{\mathbf{\Sigma}}}
% \newvariable{\TheCollapsingMap}{\pi}
% \newcommand{\TheReals}{\RRR\OptExponent}
% \newcommand{\ThePositiveReals}{\RRR^{+}}
% \newcommand{\TheNegativeReals}{\RRR^{-}}
% \newcommand{\TheComplexNumbers}{\CCC\OptExponent}
% \newcommand{\SetOfCores}[1]{\operatorname{Cores}\EvalAt{#1}}
% \newvariable{\TheCoreGraph}{C}
% \newindexedmap{\TheBordifiedProjection}{\pi}
% \newindexedmap{\TheMetricRescale}{r}
% \newvariable{\BestvinaFeighnBordification}{\overline{\OuterSpace}}
% \newvariable{\BestvinaBuxComplex}{Y}
% \newvariable{\TheOrderSimplex}{\Delta}
% \newvariable{\TheGraphMetric}{l}
% \newvariable{\TheGraphMetricFam}{\mathbf{l}}
% \newvariable{\TheHierarchyOfScales}{\mathcal{H}}
% \newvariable{\TheGraphSequence}{\mathcal{G}}
% \newvariable{\AltGraphSequence}{\mathcal{D}}
% \newvariable{\TheGraphOpenCell}{W}
% \newvariable{\TheGraphClosedCell}{\overline{\TheGraphOpenCell}}
% \newvariable{\TheGraphHomologyClass}{\nu}
% \newvariable{\TheGraphHeight}{h}
% \newvariable{\TheHomologyHeight}{\mathbf{h}}
% \newvariable{\TheBestvinaFeighnPoint}{\mathbf{x}}
% 
% %
% % Rooted Trees
% %
% \newcommand{\geomprod}{\otimes}
% \newcommand{\GrigorchukGroup}{\mathcal{G}\OptIndexOptPar}
% \newvariable{\GriCover}{\Gamma}
% \newmap{\GriPush}{\Phi}
% \newvariable{\TheTreeLevel}{n}
% \newvariable{\TheFirstGrigorchuk}{\GrigorchukGroup[\One]}
% \newindexedmap{\TheRootedTree}{T^{\bullet}}
% \newvariable{\TheLeftSubtree}{T^{\mathrm{l}}}
% \newvariable{\TheRightSubtree}{T^{\mathrm{r}}}
% \newvariable{\TheRootedTreeAut}{\mathcal{T}^{\bullet}}
% \newindexedmap{\TheRootedTreeProjection}{\pi}
% \newcommand{\TheTreeStabilizer}{\mathcal{T}_{\Two}\OptParentheses}
% \newvariable{\TheLRTreeSubgroup}{\TheTreeStabilizer[\One]}
% \newvariable{\TheTreeAutGroup}{A}
% \newvariable{\AltTreeAutGroup}{B}
% \newindexedmap{\TreeSwap}{\sigma}
% \newvariable{\TheZTwoElement}{\varepsilon}
% %\newvariable{\TheTreeAutomorphism}{\psi}
% \newvariable{\GriOne}{\beta}
% \newvariable{\GriTwo}{\gamma}
% \newvariable{\GriThree}{\delta}
% \newindexedmap{\Count}{C}
% \newcommand{\ComplexityOf}{C\EvalAt}
% \newcommand{\GriCompl}[4]{\left[#1;#2,#3,#4\right]}
% \newvariable{\TheGrigorchukElement}{\xi}
% \newvariable{\AltGrigorchukElement}{\zeta}
% \newvariable{\ThirdGrigorchukElement}{\chi}
% 
% \newvariable{\ConjugatorClasses}{Q}
% 
% \newindexedmap{\GriTreeProj}{\pi}
% 
% \newvariable{\GriT}{t}
% \newvariable{\GriU}{u}
% \newvariable{\GriV}{v}
% \newvariable{\GriW}{w}
% \newvariable{\GriB}{B}
% \newvariable{\GriK}{K}
% \newvariable{\GriKElement}{\kappa}
% \newvariable{\GriD}{D}
% \newvariable{\SwapSubstitute}{\tilde{\TreeSwap}}
% \newvariable{\GriBasicCommutator}{\xi}
% \newvariable{\TheReductionCount}{r}
% 
% \newindexedmap{\GriCoverSquare}{\psi}
% 
% %
% % Finite State Automata
% %
% \newvariable{\TheAutomaton}{A}
% \newvariable{\AltAutomaton}{B}
% \newvariable{\TheSetOfStatePairs}{\mathcal{P}}
% \newvariable{\TheState}{S}
% \newvariable{\AltState}{T}
% \newindexedmap{\TheStringTransformation}{\varphi}
% \newindexedmap{\AltStringTransformation}{\psi}
% 
% %
% % Amenability
% %
% \newvariable{\ClassElementaryAmenable}{EG}
% \newvariable{\ClassAmenable}{AG}
% \newvariable{\ClassNoFreeSubgr}{NF}
% \newvariable{\TheClass}{\mathcal{C}}
% \newvariable{\TheOrdinal}{\alpha}
% \newvariable{\AltOrdinal}{\beta}
% 
% \newvariable{\TheRobotSet}{\mathcal{R}}
% \newvariable{\TheRobot}{R}
% \newvariable{\TheRobotPath}{\sigma}
% \newvariable{\StartingRobotsNumber}{N_0}
% \newvariable{\EndingRobotsNumber}{N_1}
% 
% %
% % Linear Algebra
% %
% \newvariable{\TheEigenvalue}{\lambda}
% \newcommand{\ProjSpaceOf}[1][]{
%   \PPP^{#1}\EvalAt
% }
% \newcommand{\AmericanProjOf}[2][]{#2\PPP\IfNonEmpty{#1}{_#1}}
% \newvariable{\ImUnit}{\mathrm{i}}
% %\newcommand{\Det}{\operatorname{det}}
% \newcommand{\Trace}{\operatorname{tr}}
% \newcommand{\DetOf}{\Det\EvalAt}
% \newcommand{\TraceOf}{\Trace\EvalAt}
% \newvariable{\TheLinearForm}{\lambda}
% \newvariable{\TheOrderedBasis}{\mathcal{B}}
% \newvariable{\TheStandardBasis}{\mathcal{B}^*}
% 
% 
% %
% % Hyperbolic Geometry
% %
% \newcommand{\HypSpace}[1][\Two]{\HHH^{#1}}
% \newcommand{\HypPlane}{\HypSpace[\Two]}
% \newcommand{\PoincareDisk}{\DDD^{\Two}}
% \newvariable{\MatUL}{a}
% \newvariable{\MatUR}{b}
% \newvariable{\MatLL}{c}
% \newvariable{\MatLR}{d}
% \newvariable{\TheIdentityMatrix}{\III}
% \newvariable{\TheOrder}{n}
% \newvariable{\TheFundamentalDomain}{D}
% \newvariable{\SlTwoFD}{\TheFundamentalDomain}
% \newvariable{\SlTwoSD}{\ClosureOf{\SlTwoFD}}
% \newvariable{\SlTwoGS}{\TheGeneratingSet}
% \newvariable{\TheTBTMatrix}{\TwoByTwoMatrix{\MatUL}{\MatUR}{\MatLL}{\MatLR}}
% 
% %
% % Baumslag-Solitar
% %
% \newcommand{\BaumslagSolitarGroup}[1][]{%
%   BS\IfNonEmpty{#1}{\EvalAt{#1}}
% }
% \newvariable{\BaumslagSolitarGenA}{a}
% \newvariable{\BaumslagSolitarGenB}{b}
% \newvariable{\BaumslagSolitarExpN}{p}
% \newvariable{\BaumslagSolitarExpM}{q}
% 
% %
% % Manifolds
% %
% \newcommand{\DiffeomorphismGroupOf}{\operatorname{Diff}\OptExponentParentheses}
% \newcommand{\OrientedDiffeomorphismGroupOf}{\operatorname{Diff}^{\circ}\OptIndexParentheses}
% \newcommand{\SomeCoverOf}[1]{\bar{#1}}
% \newvariable{\TheManifold}{M}
% \newvariable{\AltManifold}{N}
% \newvariable{\TheCoverManifold}{\bar{\TheManifold}}
% \newvariable{\TheCoverManifoldPoint}{\bar{\TheManifoldPoint}}
% \newvariable{\TheChartDomain}{U}
% \newvariable{\TheChartRange}{\tilde{U}}
% \newvariable{\AltChartDomain}{V}
% \newvariable{\AltChartRange}{\tilde{V}}
% \newvariable{\TheCoverChartDomain}{\SomeCoverOf{\TheChartDomain}}
% \newvariable{\TheCoverChartMap}{\SomeCoverOf{\TheChartMap}}
% \newvariable{\TheChartMap}{\varphi}
% \newvariable{\TheChartLift}{\tilde{\TheChartMap}}
% \newvariable{\AltChartMap}{\psi}
% \newvariable{\TheCoordinateChange}{\xi}
% \newvariable{\TheModelManifold}{\mathcal{X}}
% \newvariable{\TheStructureGroup}{\mathcal{I}}
% \newvariable{\AltStructureGroup}{\mathcal{H}}
% \newvariable{\TheModelPoint}{x}
% \newvariable{\TheStructureHomeo}{\xi}
% \newvariable{\AltStructureHomeo}{\zeta}
% \newvariable{\ThirdStructureHomeo}{\chi}
% \newvariable{\TheManifoldPoint}{P}
% \newvariable{\AltManifoldPoint}{Q}
% \newvariable{\TheManifoldBasePoint}{\underbar{\TheManifoldPoint}}
% \newvariable{\TheGeometricStructure}{\mathcal{G}}
% \newvariable{\TheGeometricMap}{\nu}
% 
% \newcommand{\TheStructure}{\Pair{\TheStructureGroup}{\TheModelManifold}}
% \newcommand{\AltStructure}{\Pair{\AltStructureGroup}{\TheModelManifold}}
% 
% \newvariable{\TheEuclStructure}{\mathcal{E}}
% \newvariable{\TheHyperbolicStructure}{\mathcal{H}}
% 
% \newvariable{\TheJordanDomain}{J}
% \newvariable{\AltJordanDomain}{J^*}
% \newvariable{\AltJordanIntersectionSet}{M}
% \newvariable{\AltJordanBoundarySet}{B}
% \newvariable{\TheRectangle}{R}
% \newparexpvar{\TheJordanPolygon}{P}
% \newvariable{\TheEuclideanPoint}{x}
% 
% \newvariable{\TheDevelopingMap}{\delta}
% 
% \newvariable{\TeichmSpace}{\mathcal{T}}
% \newvariable{\ModuliSpace}{\mathcal{M}}
% \newvariable{\DeformationSpace}{\mathcal{D}}
% \newcommand{\HomeosOf}{\mathrm{Homeo}\OptIndexParentheses}
% \newcommand{\EuclStructuresOf}{\mathcal{E}\OptIndexParentheses}
% \newcommand{\SimStructuresOf}{\mathcal{S}\OptIndexParentheses}
% \newcommand{\HypStructuresOf}{\mathcal{H}\OptIndexParentheses}
% \newcommand{\IsomOf}{\mathrm{Isom}\OptIndexParentheses}
% %\newvariable{\TheIsometry}{\iota}
% \newcommand{\SimOf}{\mathrm{Sim}\OptIndexParentheses}
% %\newvariable{\TheSimilarity}{\sigma}
% \newvariable{\TheDeckTransformation}{\tau}
% \newcommand{\IDHom}{\Hom^{\text{i,d}}}
% \newcommand{\IDHomFromTo}{\IDHom\OptIndexDoubleArg}
% \newcommand{\HomFromTo}{\Hom\OptIndexDoubleArg}
% 
% %
% % Surfaces
% %
% \newvariable{\DehnNielsenMap}{\nu}
% \newvariable{\AltDehnNielsenMap}{\tilde\nu}
% 
% \newvariable{\TheCoverHomeomorphism}{\UniversalCoverOf{\TheHomeomorphism}}
% \newvariable{\AltCoverHomeomorphism}{\UniversalCoverOf{\AltHomeomorphism}}
% 
% \newvariable{\TheTorusCover}{\UniversalCoverOf{\TheTorus}}
% \newvariable{\TheTorusCoverBasePoint}{\UniversalCoverOf{\TheTorusBasePoint}}
% \newvariable{\TheTorusCoverHomeomorphism}{\TheCoverHomeomorphism}
% \newvariable{\TheTorusHomeomorphism}{\TheHomeomorphism}
% \newvariable{\TheLoop}{\gamma}
% \newvariable{\AltLoop}{\TheLoop'}
% \newvariable{\TheLoopLift}{\UniversalCoverOf{\TheLoop}}
% \newvariable{\TheHolonomy}{\eta}
% \renewcommand{\TheHolonomyOf}{\TheHolonomy\thinspace\OptIndexParentheses}
% \newvariable{\TheDeformation}{\Psi}
% \newvariable{\LengthSpectrum}{\Sigma}
% \newvariable{\TheCurveSystem}{\Delta}
% 
% \newvariable{\TheColor}{a}
% \newvariable{\AltColor}{b}
% \newvariable{\ThirdColor}{c}
% \newvariable{\ThePositiveArc}{A^+}
% \newvariable{\TheNegativeArc}{A^-}
% 
% \newvariable{\ThePolygonDiagram}{D}
% \newvariable{\ThePolygonTile}{\CoverOf{\ThePolygonDiagram}}
% \newvariable{\TheOpenPolygonTile}{\ThePolygonDiagram^{(2)}}
% \newvariable{\TheOpenEdgeNbhd}{\ThePolygonDiagram^{(1)}}
% \newvariable{\TheOpenVertexNbhd}{\ThePolygonDiagram^{(0)}}
% 
% \newvariable{\TheHomotopyEquivalence}{\TheMap}
% \newvariable{\AltHomotopyEquivalence}{\AltMap}
% \newvariable{\TheHomotopyEquivalenceCover}{\UniversalCoverOf{\TheHomotopyEquivalence}}
% 
% \newvariable{\TheSurfaceHomotopyEquivalence}{\TheMap}
% \newvariable{\AltSurfaceHomotopyEquivalence}{\AltMap}
% \newvariable{\TheSurfaceHomotopyEquivalenceCover}{\UniversalCoverOf{\TheSurfaceHomotopyEquivalence}}
% 
% \newvariable{\TheSurfaceHomeomorphism}{\TheHomeomorphism}
% \newvariable{\TheSurfaceUnivCoverHomeomorphism}{\TheCoverHomeomorphism}
% 
% \newvariable{\SurfaceOuterIsomorphism}{\Phi}
% 
% \newvariable{\TheHypWidth}{\eta}
% 
% \newvariable{\TheClosedGeodesics}{\Gamma}
% 
% \newvariable{\TheSurfacePointSet}{\mathcal{P}}
% 
% 
% %
% % HNN
% %
% \newvariable{\TheStableLetter}{t}
% \newvariable{\AltStableLetter}{s}
% 
% 
% %
% % Coxeter Groups / Artin Groups
% %
% \newvariable{\TheCoxeterGroup}{W}
% \newvariable{\TheCoxeterGeneratingSet}{S}
% \newvariable{\TheCoxeterGenerator}{s}
% \newvariable{\AltCoxeterGenerator}{t}
% \newvariable{\TheCoxeterGroupElement}{w}
% \newvariable{\TheCoxeterMatrix}{M}
% \newvariable{\TheCoxeterCoefficient}{m}
% \newcommand{\TheCoxeterMatrixEntry}[2]{\TheCoxeterCoefficient_{#1,#2}}
% 
% \newvariable{\TheHyperplaneSet}{\mathcal{H}}
% \newvariable{\TheHyperplane}{H}
% \newvariable{\TheReflection}{\rho}
% 
% \newvariable{\TheWall}{H}
% 
% \newvariable{\TheChamber}{C}
% \newvariable{\AltChamber}{D}
% \newvariable{\TheFundamentalChamber}{\TheChamber^{*}}
% 
% \newvariable{\TheCoxeterWord}{\underbar{\TheCoxeterGenerator}}
% \newvariable{\AltCoxeterWord}{\underbar{\AltCoxeterGenerator}}
% 
% \newcommand{\CoxeterSupportOf}[1]{\left|#1\right|}
% \newcommand{\isAdjacent}[1][]{
%   \IfEmptyThenElse{#1}{%
%     |%
%   }{%
%     |_{#1}%
%   }
% }
% \newcommand{\GallerySep}{\isAdjacent}
% \newvariable{\CoxeterDistance}{\delta}
% \renewcommand{\CoxeterDistanceOf}[2]{\delta\left(#1,#2\right)}
% 
% \newcommand{\HitsOf}[2]{\operatorname{hits}\left(#1,#2\right)}
% 
% \newcommand{\opposite}{\longleftrightarrow}
% 
% \newvariable{\TheChamberSystem}{\mathcal{C}}
% \newvariable{\TheGallery}{\mathbf{g}}
% 
% \newvariable{\TheCoxeterSubset}{J}
% \newvariable{\AltCoxeterSubset}{I}
% \newvariable{\TheCoxeterPolyhedron}{P}
% \newvariable{\TheMoussongComplex}{X}
% \newvariable{\TheMoussongLink}{L}
% 
% \newvariable{\TheResidue}{c}
% \newvariable{\AltResidue}{d}
% \newvariable{\WallsThrough}{\TheHyperplaneSet}
% 
% \newvariable{\TheFolding}{f}
% \newvariable{\AltFolding}{f'}
% \newvariable{\TheRoot}{\alpha}
% 
% \newvariable{\ThePosHalfspace}{U^+}
% \newvariable{\TheNegHalfspace}{U^-}
% \newvariable{\TheTitsCone}{C}
% \newvariable{\TheGeometricRepresentation}{\rho}
% \newvariable{\TheTitsRepresentation}{\tau}
% 
% \newvariable{\TheArtinGroup}{A}
% \newvariable{\ThePureArtinGroup}{P}
% \newvariable{\TheArtinGeneratingSet}{\TheCoxeterGeneratingSet}
% \newvariable{\TheArtinSubset}{\TheCoxeterSubset}
% \newvariable{\TheArtinGenerator}{\TheCoxeterGenerator}
% \newvariable{\AltArtinGenerator}{\AltCoxeterGenerator}
% 
% \newvariable{\Blue}{\mathbf{b}}
% \newvariable{\Green}{\mathbf{g}}
% \newvariable{\Red}{\mathbf{r}}
% 
% \newvariable{\ThePunctureSet}{P}
% \newvariable{\ThePunctureNum}{m}
% 
% \newvariable{\SalvettiCover}{Y}
% \newvariable{\SmallArtinPoset}{\mathcal{A}}
% \newvariable{\EnlargedSmallArtinPoset}{\SmallArtinPoset^{-}}
% \newvariable{\TheDavisCorner}{D}
% \newvariable{\TheConvexSet}{C}
% 
% \newvariable{\TheGraphGroup}{G}
% \newvariable{\TheBestvinaBradyGroup}{K}
% \newvariable{\TheBestvinaBradyComplex}{Q}
% \newvariable{\TheBestvinaBradyCover}{X}
% 
% \newvariable{\TheBestvinaBradyMap}{h}
% \newvariable{\TheBestvinaBradyLift}{h}
% 
\newvariable{\ForestComplex}{\mathcal{F}}
% \newvariable{\TheStallingsSet}{S}
% 
% \newvariable{\TheBound}{N}
% 
% 
% %
% % Outer Space
% %
% \newvariable{\TheMarking}{\mu}
% \newvariable{\TheLabelling}{\lambda}
% \newvariable{\TheCollaps}{c}
% 
% \newvariable{\TheMetricGraph}{\underline{\TheGraph}}
% \newvariable{\AltMetricGraph}{\underline{\AltGraph}}
% \newvariable{\ThePiecewiseIsometry}{\varphi}
% \newvariable{\AltPiecewiseIsometry}{\psi}
% 
% \newvariable{\TheSphereComplex}{\overline{\OuterSpace}}
% \newvariable{\TheSphereSetComplex}{X}
% \newvariable{\TheSphereSystemComplex}{Y}
% \newvariable{\TheSphereSystem}{\mathcal{S}}
% \newvariable{\AltSphereSystem}{\TheSphereSystem'}
% \newvariable{\TheSimpleSphereSystem}{\underline{\TheSphereSystem}}
% \newvariable{\AltSimpleSphereSystem}{\TheSimpleSphereSystem'}
% \newvariable{\TheSimpleSphereSystemComplex}{X}
% 
% \newvariable{\TheSphereSet}{S}
% \newcommand{\EnlargementOf}[1]{\overline{#1}}
% \newvariable{\TheEnlargedSphereSet}{\EnlargementOf{\TheSphereSet}}
% 
% \newvariable{\TheSimpleSphere}{\underline{\TheSphere}}
% \newvariable{\AltSimpleSphere}{\underline{\AltSphere}}
% \newvariable{\TheSphereSystemDifference}{\Delta}
% \newvariable{\TheTriangulatedSimplex}{T}
% 
% \newvariable{\TheComplementaryComponent}{P}
% 
% \newvariable{\TheGerstenObstruction}{H}
% \newvariable{\TheGerstenEmbedding}{\iota}
% \newvariable{\TheGerstenHomomorphism}{\varphi}
% 
% 
% 
%
% Braid Posets
%
\newvariable{\TheBraidsPoset}{\mathcal{B}}
\newvariable{\TheBotNumber}{n}
\newvariable{\TheTopNumber}{m}
\newvariable{\TheBarNumber}{k}
\newvariable{\TheGraphFam}{\mathcal{G}}
\newvariable{\GraphPoset}{P}
\newvariable{\GraphComplex}{C}
\newvariable{\TanglePoset}{\GraphPoset^{\mathrm{tn}}}
\newvariable{\TangleComplex}{\GraphComplex^{\mathrm{tn}}}
\newvariable{\ChessboardPoset}{\mathrm{CBP}}
\newvariable{\ChessboardComplex}{\mathrm{CBC}}
\newvariable{\MatchingPoset}{\mathrm{MP}}
\newvariable{\MatchingComplex}{\mathrm{MC}}
\newvariable{\Matchings}{\mathcal{M}}
\newvariable{\SubGraphs}{\mathcal{S}}

\newvariable{\PinchedBraidPoset}{X}
\newvariable{\PinchedBraidComplex}{X}
\newvariable{\TheTopSlot}{\mathrm{top}}
\newvariable{\TheBotSlot}{\mathrm{bot}}
\newvariable{\TheStrand}{s}
\newvariable{\TheCutOutGraph}{\Theta}
% 
% %
% % Subgroup Posets
% %
\newvariable{\ElementaryAbelianSubgroupPoset}{\mathcal{A}}
% \newvariable{\BrownPoset}{\mathcal{S}}
% \newvariable{\BrownComplex}{S}
% \newvariable{\ThePSubgroup}{P}
% 
% %
% % Bass-Serre Theory
% %
% \newvariable{\TheVertexGroup}{\mathcal{G}}
% \newcommand{\TheEdgeGroup}{\TheVertexGroup}
% \newvariable{\TheEdgeHom}{\iota}
% \newvariable{\TheVertexSpace}{\mathcal{X}}
% \newcommand{\TheEdgeSpace}{\TheVertexSpace}
% \newcommand{\AltVertexSpace}{\AltSpace}
% \newcommand{\AltEdgeSpace}{\AltSpace}
% \newvariable{\TheEdgeMap}{\TheMap}
% \newvariable{\TheGroupsGraph}{\mathcal{G}}
% \newvariable{\TheSpacesGraph}{\mathcal{X}}
% \newvariable{\AltSpacesGraph}{\mathcal{Y}}
% \newvariable{\TheMappingCylinder}{M}
% \newvariable{\TheGraphProjection}{\pi}
% \newvariable{\TheThickSpace}{X}
% \newvariable{\TheConnectionSpace}{Y}
% \newvariable{\TheThickCover}{\CoverOf{\TheThickSpace}}
% 
% %
% % Buildings
% %
% \newvariable{\AffBuild}{X}
% \newvariable{\AffBuildProd}{\mathbf{\AffBuild}}
% 
% 
% \endinput
% 

